The Optimal Error Resilience of Interactive Communication Over Binary Channels

In interactive coding, Alice and Bob wish to compute some function $f$ of their individual private inputs $x$ and $y$. They do this by engaging in a non-adaptive (fixed order, fixed length) protocol to jointly compute $f(x,y)$. The goal is to do this in an error-resilient way, such that even given some fraction of adversarial corruptions to the protocol, both parties still learn $f(x,y)$. In this work, we study the optimal error resilience of such a protocol in the face of adversarial bit flip or erasures. While the optimal error resilience of such a protocol over a large alphabet is well understood, the situation over the binary alphabet has remained open. In this work, we resolve this problem of determining the optimal error resilience over binary channels. In particular, we construct protocols achieving $\frac16$ error resilience over the binary bit flip channel and $\frac12$ error resilience over the binary erasure channel, for both of which matching upper bounds are known. We remark that the communication complexity of our binary bit flip protocol is polynomial in the size of the inputs, and the communication complexity of our binary erasure protocol is linear in the size of the minimal noiseless protocol computing $f$.

==> erasure/1.2-outline.tex <==
\rnote{i kinda feel like this should go back in the section; and we should write a more high level overview of the $\frac12$ protocol}
For clarity, we describe the first few rounds of the protocol.
\begin{enumerate}
    \item 

        Alice begins the protocol in $\speaker$ mode with her first bit as the noiseless transcipt, and Bob begins the protocol in $\listener$ mode with an empty transcript. Alice tries to communicate the first message $\pi_1 \in \{ 0, 1 \}$ of $\pi$ to Bob by sending over the bits of $c(\pi_1)$ to Bob, \ynote{need to define $c$ since the reader will read this before reading the formal description} repeating a bit until she receives a $1$ from him. She then sends $1$'s for the rest of the block. If she received confirmation bits from Bob for the entirety of $c(\pi_1)$, she switches to $\passer$ mode at the end of block $1$. Note that Bob remains in $\listener$ mode for the duration of block $1$, since the first message he receives from Alice must be a $1$.  \ynote{Again, this last sentence is not self contained.}
        
    \item 
        If Alice did not receive both confirmation bits from Bob, she is still in $\speaker$ mode at the beginning of block $2$. The parties rerun block $1$, with Alice trying to communicate $\pi_1$ from scratch.
        
        If Alice did receive both confirmation bits from Bob, she is now in $\passer$ mode at the beginning of block $2$. She sends $0$'s until she receives a $1$, at which point she switches to $\listener$ mode, sending a $1$ everytime she receives a message (including the recently received $1$) and a $0$ otherwise. Bob begins the block in $\listener$ mode: then, as the first message he receives from Alice in the block is a $0$, he switches to $\speaker$ mode and tries to communicate $\pi_2$ to Alice (beginning with sending a $1$, which is the first bit of $c(\pi_2)$, immediately after the most recently received $0$). Note that if Alice does not receive any of Bob's $1$'s for some rounds, she continues to send $0$ by default (as she is still in $\passer$ mode), which coincides with her behavior if she were in $\listener$ mode. Eventually, if/when Alice receives a $1$, she switches to being in $\listener$ mode, and for the rest of the block Bob is the $\speaker$ trying to communicate $\pi_2$ to Alice. We point out that here, the roles of $\speaker$ and $\listener$ have been reversed.
    \item 
        Round $3$ can start with Alice and Bob in any of the following pairs of roles: $(\speaker, \listener)$, $(\passer, \listener)$, $(\passer, \speaker)$, $(\listener, \speaker)$. We've already described the interactions in the $(\speaker, \listener)$ and $(\passer, \listener)$ scenarios ($(\listener, \speaker)$ works symmetrically), so it remains to describe the $(\passer, \speaker)$ scenario. In this case, Alice sends $0$'s until she receives a $1$. Meanwhile, Bob sends $1$'s (since a $1$ is the first bit of $c(\pi_2)$) until he receives a $1$. We've already pointed out that Alice's behavior as $\passer$ and with Bob as $\speaker$ is equivalent to if she were in the $\listener$ role. Furthermore, Alice becomes $\listener$ as soon as she hears a $1$, so Bob cannot move onto the next bit of $c(\pi_2)$ before Alice becomes a listener. From this point on, their behavior is the same as in the $(\listener, \speaker)$ scenario.
    \item 
        In general, in block $j$, Alice and Bob can be in any two different roles (Claim~\ref{claim:modes}), with behavior as described above.
\end{enumerate}

==> intro/intro-old.tex <==
Interactive coding is an interactive analogue of error correcting codes \cite{Shannon48, Hamming50}, which was introduced in the  seminal work of Schulman~\cite{Schulman92,Schulman93,Schulman96}, and has been an active area of study since. While error correcting codes address the problem of sending a {\em message} in a way that is resilient to error, interactive coding addresses the problem of   converting an {\em interactive protocol} to an error resilient one.

Suppose two parties, Alice and Bob, each with a private input,  engage in a protocol~$\Pi$ to jointly compute a function $f$ of their private inputs.   {\em Given such a protocol $\Pi$, can we design a protocol~$\Pi'$ that  computes $f$ and at the same time is resilient to adversarial errors?} 
%More specifically, Alice and Bob engage in a fixed length, fixed order of speaking (nonadaptive) protocol, and output the function $f$ at the end. Can they be resilient to a constant fraction of the total communication being corrupted?
Schulman~\cite{Schulman96} answered the question in the affirmative, presenting a scheme that is resilient to $\frac{1}{240}$ adversarial corruptions (bit flips) over a binary channel with a constant information rate.\footnote{Constant information rate means that the error-resilient protocol incurs only a  constant multiplicative overhead to the communication complexity.} %\rnote{we need to define rate at some point} 
This work begs the following natural question: {\em what is the optimal error resilience possible?}   This is precisely the focus of our work.

% Throughout this work, we only consider protocols of fixed length and non-adaptive speaking order (where the adversary cannot cause an ambiguity as to which party speaks next). The reason is that any form of adaptivity in this setting (either in the protocol length or in the speaking order) renders itself to various possible definitions of  error rate, which results from the fact that the adversary can influence the number of messages sent.  Rather, we focus on the non-adaptive case where the number of bits sent is fixed and hence the definition of error rate is simply the number of errors divided by the fixed number of bits exhanged. \rnote{do we want this paragraph?}

Two natural types of corruption to consider are toggle (where the adversary can replace a symbol with one of their choice) and erasure (where the adversary can replace a symbol with $\perp$).
In both of these settings, there are known protocols that achieve optimal error resilience for large constant-sized alphabets. In the toggle setting, Braverman and Rao~\cite{BravermanR11} constructed a protocol which achieves the optimal error resilience of $\frac14$.  In the erasure setting, 
% the optimal error resilence (over large constant size alphabet) is known to be $\frac12$, achieved by~
\cite{FranklinGOS15,EfremenkoGH16} constructed protocols achieving error resiliencce $\frac12$. Corresponding impossibility bounds are known \cite{ghaffariH14,FranklinGOS15}.

However, despite much effort, the optimal error resilience for both types of corruption over a \emph{binary} alphabet is still unknown. 
For both types of corruption, a protocol achieving error resilience of $r$ over a large alphabet trivially translates to a protocol over a binary alphabet with error resilience of $\frac{r}2$ by replacing every letter of the large alphabet with an binary error correcting code of relative distance $\frac12$. Thus, the results of~\cite{BravermanR11,FranklinGOS15} give protocols that achieve error resilience $\frac18$ over the binary toggle channel and $\frac14$ over the binary erasure channel. Unfortunately, the corresponding impossibility bounds \cite{BravermanR11, FranklinGOS15} for large alphabets do not lead to matching impossibility bounds in the binary case. Over the binary toggle channel, the best known impossibility bound is $\frac16$ \cite{EfremenkoGH16}, and over the binary erasure channel, the best known impossibility bound is $\frac12$ \cite{FranklinGOS15}. Pinning down the exact constant between $\frac18$ and $\frac16$, and between $\frac14$ and $\frac12$, has been an intriguing open problem. 
% which is at the core of why resolving this question for binary alphabets is so much harder.

There has been some recent work towards this goal. Over the binary bit flip channel, \cite{EfremenkoKS20b} broke the $\frac18$ barrier for the first time, describing a protocol that achieves $\frac5{39}$ resilience to adversarial bit flips.\mnote{yael is right that we should highlight this result more} Over the binary erasure channel, \cite{EfremenkoGH16} gives a protocol achieving a $\frac13$ resilience to erasures. \rnote{i brought this paragraph back: it sounded weird to not have the complete history before we say what our result is}

In this work, we fully resolve the question of the optimal error resilience of a non-adaptive protocol over a binary alphabet. Specifically, we show that the known impossibility bounds are tight: we construct protocols achieving error resilience $\frac16$ to adversarial bit flips and $\frac12$ to adversarial erasures.

\paragraph{Binary Bit Flip Channel} \mnote{this is just a word dump, we should think about exactly what to say more. It is important that we frame the difficulties and argue that our result is "surprising" or "interesting" though.}
As indicated earlier, for a while the best known resilience over the binary bit flip channel was $\frac18$, translating from the large alphabet case. Efremenko et al. \cite{EfremenkoKS20b} even argue this is a natural barrier: the $\frac18$ comes from three separate $\frac12$ factors, each stemming from a different property that we require. The first $\frac12$ factor comes from the fact that we want a binary protocol (classical binary error correcting codes have distance approaching $\frac12$, whereas codes over a large alphabet can have distance approaching $1$). The second $\frac12$ factor comes from the requirement of unique decoding (the adversary can corrupt a message to be halfway between two codewords). The last $\frac12$ factor comes from the fact that the message exchange task, like all interactive tasks, is ‘two-sided’, and in order to fail the task, the adversary only needs to corrupt the weaker of the two parties.

They then show that despite the fact that designing a protocol with any two of the three required properties can only achieve $\frac14$ error resilience, the $\frac18$ barrier does not actually hold for all three! They design a protocol that achieves $\frac5{39}$ error resilience, which is slightly greater than $\frac12$. So what is the actual barrier? and is there a framing that justifies it? As stated earlier, in this paper we show the barrier is $\frac16$.

Another way of looking at the problem is the following. There is a well known result\cite{SpencerW92} that if Alice is trying to send Bob an input $x$ and receives full feedback about which of her her messages are corrupted, she can be resilient to $\frac13$ bit flips. This trivially translates to a $\frac16$ error resilient protocol in binary bit flip channel under the \emph{feedback} model, by having Alice engage in this procedure first, then Bob. So now the question becomes: why might we think we can get rid of this feedback? In the solution we just proposed, Alice talks first then Bob, but the adversary only really has budget to corrupt one of them, say Alice. So then what if we intermingle Bob's messages with Alice's, and include feedback in Bob's messages? The problem is this feedback isn't actually completely reliable even though the adversary doesn't want to waste budget corrupting Bob. So now whether or not $\frac16$ is the right barrier comes down to the following question: in this setting, is noisy feedback as powerful as guaranteed noiseless feedback? Using clever techniques, we answer this question in the affirmative. \mnote{theres also one other subtlety: how to send the feedback while not messing up your own procedure of sending your input in a $\frac13$ resilient way} \mnote{mention that there has been study of noisy feedback in the past, mostly to no avail, talk about the difficulties}

\paragraph{Binary Erasure Channel.}
We first remark that $\frac12$ is the maximal possible erasure resilience of a two-party interactive protocol over \emph{any} alphabet: the adversary can simply erase all messages of the party that speaks less. 

Previous attempts to construct maximally erasure resilient interactive protocols over the binary alphabet did so by starting with such a protocol over a larger alphabet and then replacing each character with a binary error correcting code. For instance, in~\cite{EfremenkoGH16}, they constructed a protocol resilient to $\frac12$ erasures over an alphabet of size 4, then replaced the alphabet with the four strings $(000)^*, (110)^*, (101)^*, (011)^*$ that have relative distance $\frac23$. This resulted in an binary protocol resilient to $\frac12 \cdot \frac23 = \frac13$ erasures. Unfortunately, $\frac13$ is also the maximal erasure resilience attainable with this approach, as $\frac12$ is the maximal erasure resilience of a protocol over any alphabet and $>2$ binary codewords necessarily have relative distance $\le \frac23$. 

In our paper, we deviate from this strategy of substituting binary codewords for a larger alphabet.

% As mentioned earlier, when \cite{FranklinGOS15} study erasure channels, they give a $\frac12$ resilient protocol for large alphabets. This trivially translates to a $\frac14$ resilient protocol over the binary channels, \cite{EfremenkoGH16} reduce the size of this large alphabet to one of size only $4$. This actually translates to a $\frac13$ resilient scheme, because $4$ codewords can be made distance $\frac23$ instead of distance $\frac12$ in the binary alphabet. However, the question of whether this barrier is actually solid has remained open. In the bit flip channel, binary is in fact a factor of $\frac23$ less error resilient than large alphabet. As such, the natural barrier of $\frac12\cdot\frac23$ might actually be tight.\mnote{can we find work attempting this?} It would be very surprising if binary alphabets are actually as powerful as arbitrarily large constant sized ones. Yet, in this work we answer that question in the affirmitive. 
\mnote{we should probably cite https://arxiv.org/pdf/1811.02527.pdf somewhere} 

\subsection{Our Results}

\paragraph{Over the Binary Bit Flip Channel.}

The goal of the \emph{message exchange task} is for Alice and Bob to communicate to each other their own private input. In this paper, we resolve the optimal error resilience of the message exchange task over the adversarial binary bit flip channel. 

% Alice to communicate to Bob her private input $x$ and for Bob to communicate to Alice his private input $y$. 

% To state our result in the bit flip setting, we focus on the \emph{message exchange task} where the function Alice and Bob compute is $f(x,y)=(x,y)$. The corresponding $\pi_0$ is a protocol where Alice Bob her input, then Bob sends Alice his input.

\begin{theorem}
    There exists a non-adaptive interactive protocol resilient to $\frac16 - \epsilon$ adversarial bit flips for the message exchange task. For inputs of size $n$, the communication complexity is $O_\epsilon(n^2)$, the run time of the parties is $C(\epsilon)n^{O(1)}$ for some constant $C(\epsilon)$, and the probability of success is $1-2\exp(-\Omega(\epsilon n))$.
\end{theorem}

We remark that an error resilience of $\frac16$ is in fact optimal \cite{ghaffariH14}.

We note that a noise resilient protocol for the message exchange task implies the same noise resilience for general interactive coding, since the parties can simply exchange their entire inputs and compute the function separately. However, this may result in an exponential blowup in communication complexity relative to a corresponding error-free protocol $\pi_0$ for simpler functions they might want to compute. We leave it as an open problem to achieve $\left(\frac16-\epsilon\right)$ error resilience with a protocol whose communication complexity and run time is polynomial in $|\pi_0|$ or ideally even linear.

\paragraph{Over the Binary Erasure Channel.}

A nonadaptive interactive protocol, defined formally in Definition~\ref{def:ip}, is a procedure where Alice and Bob jointly compute a public function $f(x,y)$ of their respective private inputs $x,y\in\{0,1\}^n$. Usually, to define a protocol $\pi$ resilient to $\alpha$ fraction of corruption computing $f(x,y)$, one will start with a protocol $\pi_0$ that computes $f(x,y)$ and provide an error resilient protocol $\pi$ that computes $f(x,y)$ while retaining the efficiency of $\pi_0$.

\begin{theorem}
    For any interactive protocol $\pi_0$ of length $|\pi_0|$ computing a function $f(x,y)$ of Alice and Bob's inputs $x,y\in\{0,1\}^n$, there exists a non-adaptive interactive protocol $\pi$ resilient to $\frac12 - \epsilon$ adversarial erasures that also computes $f(x,y)$. The communication complexity and run time for each party are both $O_\epsilon(|\pi_0|)$.
\end{theorem}

As stated earlier, $\frac12$ is the highest erasure resilience one can hope to design a protocol for, so this result is optimal.


==> intro/overview-2.tex <==
\section{Technical Overview}\label{sec:overview}

We now give an overview of our two protocols achieving maximal error resilience over the binary bit flip channel and binary erasure channel respectively.

\subsection{Our Binary Protocol Resilient to $\frac16$ Bit Flips} \label{sec:overview-1/6}

We begin with the following (flawed) approach, which achieves an error resilience of $\frac18$: Alice sends an error correcting code $\ECC(x)$, and Bob sends $\ECC(y)$. Since $\ECC$ has a minimum relative distance of at most $\frac12$, the adversary can simply flip $\frac14$ of the bits of the party that speaks less so that the other party cannot distinguish between two inputs.

Recall that the maximum error resilience of any binary two-party protocol is $\frac16$ of the total communication, or $\frac13$ of either party's communication. The above flawed protocol only had error resilience of $\frac14$ of either party's communication. In order to increase this to $\frac13$ for one of the parties, we introduce a new \emph{question-answer} approach: in each round of interaction, Alice asks a question (encoded with an $\ECC$) about Bob's input, and then Bob responds with one of \emph{four} answers. 

That is, Alice keeps track of a guess $\hat{y}$ for Bob's input $y$, initially set to $\emptyset$. Each round, she sends $\hat{y}$ to Bob as her question, who responds with one of four operations to do to $\hat{y}$ as his answer: append 0 ($0$), append 1 ($1$), delete the last bit ($\rewind$), or ``bingo -- you got it right!'' ($\bullet$). These four responses allow Alice to either adjust $\hat{y}$ to be one character closer to Bob's input $y$, or build confidence that her current guess $\hat{y}$ is correct. If the adversary corrupts the response to be wrong, then Alice will get one character or confidence further from the correct $y$ \mnote{this sentence doesn't parse. we also don't account for increasing/lowering confidence in an incorrect y. actually, we also don't mention c_A here, which we kind of need to}. Then, as long as Alice receives Bob's correct answer at least $|y|$ times more than she receives a wrong answer, she will output the correct answer. The key point is that these four responses from Bob can have distance $\frac23$. Now, if the adversary simply corrupts Bob's answers, she'd have to corrupt $\approx \frac12 \cdot \frac23 = \frac13$ of Bob's rounds. 

While this achieves $\frac13$ resilience for Bob's communication, Alice's communication is still only $\frac14$-error resilient as she is sending an error correcting code. In order to attain $\frac13$ error resilience for \emph{both} parties, both parties will need to \emph{simultaneously ask and answer a question} each round.

Specifically, Alice and Bob each keep track of a guess $\hat{y}$ or $\hat{x}$ respectively for the other party's input, as well as a counter $c_A$ or $c_B$ respectively that indicates how many times they've received the ``bingo'' message for their current guess $\hat{y}$ or $\hat{x}$. If they receive the instruction $\bullet$, they increase $c_A$ or $c_B$ by $1$. Otherwise, they either decrease $c_A$ by $1$ or, if $c_A = 0$, adjust $\hat{y}$ or $\hat{x}$ by one character according to $\delta \in \{ 0, 1, \rewind \}$. At first, $\hat{y} = \hat{x} = \emptyset$ and $c_A = c_B = 0$. \mnote{this paragraph is quite redundant with the above}

Each round, Alice sends $\ECC(\hat{y}, x^*, \delta)$, where $x^*$ is the question she just heard from Bob and $\delta$ is the instruction that brings $x^*$ one character closer to her input $x$ (or $\bullet$ if $x^*=x$). Similarly, Bob sends $\ECC(\hat{x}, y^*, \delta)$. When Alice receives the message $\ECC(x^*, y^*, \delta^*)$ from Bob, she only updates $\hat{y}$ according to the direction $\delta^*$ if $y^* = \hat{y}$. Otherwise, she does nothing. Bob does the same.

% , in which case if $c_A = 0$ she adjusts $\hat{y}$ by a character corresponding to the instructions $0$, $1$, or $\rewind$, or if $c_A > 0$ she increases or decreases $c_A$ by $1$ corresponding to $\delta^* = \bullet$ or $\delta^* = 0,1,\rewind$, respectively. 

% If she receives $0$, $1$, or $\rewind$, she adjusts $\hat{y}$ by a character if $c_A = 0$ or she decreases $c_A$ by $1$. If she receives $\bullet$, she increases $c_A$ by $1$. Bob does the same.

% Each round, Alice sends $\hat{y}$ to Bob, asking for one of the four operations $0,1,\rewind,\bullet$ to do to $(\hat{y}, c_A)$. She receives $\delta^*$ as the instruction and $y^*$ indicating what Bob thought $\hat{y}$ was. She only updates if $y^*=\hat{y}$, doing the following: if $\delta^*$ is $0$, $1$, or $\rewind$, she adjusts $\hat{y}$ by a character if $c_A = 0$ and otherwise decreases $c_A$ by $1$, and if $\delta^*$ is $\bullet$, she increases $c_A$ by $1$. To engage in both question asking and answering simultaneously, Alice's full message is $\ECC(\hat{y}, x^*, \delta)$, where $\hat{y}$ is her guess, $x^*$ is the question she just heard from Bob and $\delta$ is the instruction she intends Bob to follow. Bob does the symmetric update, and sends a message of the form $\ECC(\hat{x}, y^*, \delta)$ \mnote{changed last 2 paragraphs, feel free to adjust}

%Specifically, Alice and Bob each keep track of a guess $\hat{y}$ or $\hat{x}$ respectively for the other party's input, as well as a counter $c_A$ or $c_B$ respectively that indicate how many times they've received the ``bingo'' message from the other party for their current guess $\hat{y}$ or $\hat{x}$. At first, $\hat{y} = \hat{x} = \emptyset$ and $c_A = c_B = 0$. Each round, Alice sends $\hat{y}$ to Bob, asking for one of the four operations $0,1,\rewind,\bullet$ to do to $(\hat{y}, c_A)$. If she receives $0$, $1$, or $\rewind$, she adjusts $\hat{y}$ by a character if $c_A = 0$ or she decreases $c_A$ by $1$. If she receives $\bullet$, she increases $c_A$ by $1$. Bob does the same.

%Each of Alice's messages is of the form $\ECC(\hat{y}, x^*, \delta^*)$, where $x^*$ is the question she just heard from Bob and $\delta^* \in \{ 0,1,\rewind,\bullet \}$. Likewise Bob's messages are of the form $\ECC(\hat{x}, y^*, \delta^*)$. Alice only performs an update on $\hat{y}$ if Bob's message satisfies $y^* = \hat{y}$.

The $\ECC$ we use has relative distance $\ge \frac12$ between all pairs of codewords, and for codewords of the form $\ECC(x', y', \delta_0)$ and $\ECC(x', y', \delta_1)$ with $\delta_0 \not= \delta_1$ (or equivalently $\ECC(y', x', \delta_0)$ and $\ECC(y', x', \delta_1)$ with $\delta_0 \not= \delta_1$), the codewords have relative distance $\frac23$. The idea is that if the adversary only corrupts Bob's answer, specifically only corrupting $\delta$, it will require $\approx \frac13$ corruptions of Bob's communication for Alice to output the wrong $y$.

However, it seems as if we have lost the advantage we gained earlier: the adversary can corrupt both Bob's answer $\delta$ \emph{and} his question $\hat{x}$ every other round so that Alice receives $\ECC(x', \hat{y}, \delta')$, where $x' \not= \hat{x}$ and $\delta' \not= \delta^*$. Then, every other round, Alice performs an incorrect update on $\hat{y}$ and $c_A$, so that over time she gets no closer to learning $y$. This attack only requires corrupting $\frac12$ of Bob's message every other round, for a total of $\frac14$ of his total communication.

Let us analyze this situation more closely. We count progress as the number of good updates (getting closer to the other party's input) minus the number of bad updates (getting further from the other party's input). What happens is that the adversary can corrupt $\frac12$ of Bob's message to get $-1$ progress for Alice and $0$ progress for Bob (Alice answers the wrong question for Bob so that he performs no update), from an original progress count of $(+1, +1)$ had no corruptions occurred. So, when the adversary corrupts every other of Bob's messages, Alice's progress count remains $0$, so that she cannot know $y$ at the end of the protocol. Meanwhile, Bob's progress increases at a steady rate! If there were a way to balance this, so that when Bob has made lots of progress it becomes harder to cause negative progress for Alice, perhaps we could achieve our goal of $\frac13$ error resilience for each party.

To do this, we make the following change to the way Alice and Bob make updates to their current guesses $\hat{y}$ and $\hat{x}$: they only update their respective guess $\hat{y}$ or $\hat{x}$ with probability $1$ if the question they just received is equal to their input, otherwise they update $\hat{y}$ or $\hat{x}$ with probability $0.5$. This way, when Bob has made lots of progress so that $\hat{x} = x$, if the adversary corrupts Bob's message to be $\ECC(x' \not= x, \hat{y}, \delta')$, Alice only updates $\hat{y}$ with probability $0.5$ --- this is $-0.5$ progress instead of $-1$! Now, the adversary has to corrupt two out of every three of Bob's messages in order for Alice to remain at $0$ progress, bringing us up to a $\frac13$ corruption rate for Bob's messages.

This change in update probability introduces a new situation, which is that when both Alice and Bob have made little progress, the adversary can corrupt Bob's message to be $\ECC(x \not= \hat{x}, \hat{y}, \delta')$ so that Alice performs a bad update with probability $1$, i.e. $(-1, 0)$ progress, from an original $(+0.5, +0.5)$ progress without corruption. Then, if the adversary corrupts one message every two rounds of interaction, the total progress between Alice and Bob remains $0$! To remedy this, we have Alice and Bob perform an additional update with probability $0.5$ when they see that the answer is of the form $(y^*, \bullet)$ (or $(x^*, \bullet)$) to bring their current guess $\hat{y}$ one character closer to $y^*$ (or $\hat{x}$ closer to $x^*$). Now, when Bob receives Alice's response $\ECC(\hat{y}, x, \bullet)$ to his corrupted question, he performs a $+0.5$ update, so that the total effect of the adversary's corruption to Bob's message is $(-1, +0.5)$, i.e. a $-0.5$ bad collective bad update.

It turns out this proposed algorithm works as long as Alice and Bob always receive a (possibly incorrect) codeword. We are almost done, but we need to specify their behaviors when they receive partially corrupted messages. To do this, we say that when Alice receives a message from Bob, she ``rounds'' to the nearest full codeword and does the corresponding update with some lower probability depending on the distance to the codeword. Precisely, she rounds to a codeword of the form $\ECC(x, \hat{y}, \delta)$ if the received message is relative distance $d^* < \frac13$ away, and otherwise she rounds to a codeword $\ECC(x^*, y^*, \delta^*)$ if the relative distance $d^*$ is $< \frac16$. (At most one such rounded codeword can exist since the relative distance between any two codewords is $\frac12$ and between any two of the form $\ECC(x, \hat{y}, \delta)$, varying $\delta$, it is $\frac23$.) She performs the corresponding update with probability $1 - 3d^*$ or $0.5 - 3d^*$ respectively and then replies with $\hat{y}$ and an answer to the question $\hat{x}$ or $x^*$. If no rounded codeword exists, she does no update and sends a message of the form $\ECC(\hat{y}, x, \bullet)$. 
% Under this definition of Alice and Bob's behavior, we show that $\alpha$ corruptions to a message cause on average $0.5-3\alpha$ progress to be made, so that Alice and Bob learn each others' inputs with high probability if the adversary corrupts less than $\frac16$ of the total communication.

For a formal description of the protocol and a detailed analysis, we refer the reader to Section~\ref{sec:toggle}.

% main points:
% - 1/8 is attained by ECC, ECC - bad because the adversary can corrupt 1/4 of one person
% - we instead develop question-answer paradigm - where answer is one of <=4 so answers can be 2/3 apart
% - but need to answer while also asking - say send ECC(hat{y}, x*, delta*)
% - issue is there are /many/ questions, so that distance between answers has seemingly now gone down to 1/2 again! 
% - what happens is that you can corrupt 1/2 and get (-1,0) damage, from an original (+1,+1) progress. issue is one party can be at 0 progress while the other is at + a lot -- is there a way to balance this out so that if the other party has lots of progress, then its harder to make damage to the first party? eg (-0.5, 0) from (+1, +1)
% - yes! when the other party sends hat{x} = x, then alice should update +1. if not then alice updates +0.5. 
% - new situation: the adversary can now corrupt a (+0.5, +0.5) to a (-1, 0) -- so introduce second update \bullet to correct to (-1, 0.5)


\subsection{Our Binary Protocol Resilient to $\frac12$ Erasures} \label{sec:overview-1/2}

We construct a protocol that achieves an $\frac12 - \epsilon$ erasure resilience for any $\epsilon > 0$. In our construction, we leverage a key property of the erasure channel: \emph{communication can be delayed but not wrong}. To recreate the transcript of a (w.l.o.g. alternating) noiseless protocol $\pi_0$, Alice and Bob alternate sending bits according to the following high level strategy: 

% Our goal is for Alice and Bob to recreate the transcript of a (w.l.o.g. alternating) noiseless protocol $\pi_0$. In our protocol, Alice and Bob alternate sending messages. The high level strategy is as follows:

\begin{itemize}
    \item A party (the $\speaker$) sends their next bit of $\pi_0$ \emph{until they are sure} that the other party (the $\listener$) has received their message. The $\listener$ gives feedback to the $\speaker$ by sending $0$ whenever the $\speaker$'s message was erased and $1$ whenever they receive it.
    \item The $\speaker$ signals the parties to switch roles: the $\speaker$ becomes the $\listener$ and the $\listener$ becomes the $\speaker$.
\end{itemize}

Because the adversary can only erase $\frac12-\epsilon$ of the total messages, there must be many pairs of rounds where \emph{both parties hear each other}. In each of these pairs of rounds, the $\speaker$ receives confirmation (in the form of a $1$) that the $\listener$ received the most recent message they sent. Then the two parties can unerroneously make progress in their simulation of $\pi_0$.

Intuitively, the $\speaker$ has \emph{three} things to communicate: the bit $0$, the bit $1$, and switching roles. The challenge is to do this by sending only two bits. 

We can let the bits $0$ and $1$ mean \emph{more than two things} if we let the two bits mean different things when heard at different parts of the protocol. More specifically, we partition the protocol into $\approx \frac{n}{\epsilon}$ \emph{blocks} of $\approx \frac1\epsilon$ rounds. In each block, the first bit that the $\listener$ receives ($1$ or $0$) tells them whether the $\speaker$ is trying to send a bit or switch roles. In the case that the $\speaker$ is trying to send a bit, the bits received during the rest of the block tell the $\listener$ what the $\speaker$'s bit $b$ was.

% We first describe how the $\speaker$ confirms the $\listener$ has heard their message (the next bit of $\pi_0$). The $\listener$ sends $0$ whenever they did not hear the $\speaker$'s previous message, and $1$ whenever they did. Because the adversary can only erase $\frac12-\epsilon$ fraction of the messages total, there must be many full rounds (Alice-Bob and Bob-Alice pairs) where \emph{both parties hear each other}. As such, the $\speaker$ will eventually learn that the $\listener$ heard their message.

% Now the $\speaker$ must tell the $\listener$ that it is time to switch modes. There is no easy way to do this -- if they simply use $0$ or $1$ to communicate this, the $\listener$ might believe they are only re-sending their bit, unsure about whether it was heard yet. As such, the $\speaker$ wants a third bit which signals that the $\listener$ should become a $\speaker$, which they do not have.

% Instead, the bits $0$ and $1$ will mean \emph{more than two things} when we combine them with absolute timing markers in the protocol. More specifically, we partition the protocol into $\approx \frac{n}{\epsilon}$ \emph{blocks} of $\approx \frac1\epsilon$ rounds, and the $\listener$ uses the first bit they receive in a block to inform them how to interpret the next bit in the block. Blocks will be the new unit of communication, rather than a single Alice-Bob or Bob-Alice round.

% Instead, the unit of communication will not be a single bit -- it will be a block of $\approx \frac1\epsilon$ alternating Alice and Bob messages. The $\speaker$ will use the block to send potentially a pair of bits, rather than a single bit. \mnote{alternate version of the intuition for blocks; presents some issues though so im inclined to stick with the first.}

\begin{itemize}
    \item In each block, if the $\speaker$ wants to send a bit $b$ to add to the transcript, they send $1$'s until they receive signal that the listener has heard it, at which point they send $b$ for the rest of the block.
    \item When they hear that the $\listener$ received the message $b$, they change strategies in the next block to signal the role switch: they send only $0$'s. For distinction, this version of $\speaker$ mode is called the $\passer$ mode.
    \item When the $\listener$ hears this $0$, i.e. the first message they receive in a block is a $0$, they know that they've received the bit $b$. To figure out what $b$ was, they look back at the last block where the first message they heard was $1$, and let $b=0$ if it was followed by any $0$'s and $b=1$ otherwise. Take note of a subtlety here -- the $\listener$ could have received more than one $1$ before the bit $b$, but this doesn't actually matter as they receive any $0$'s in the block if and only if $b=0$. 
    \item The $\passer$ (ex-$\speaker$) stays in $\passer$ mode, sending only $0$'s, until they hear a $1$ from the other party. This received $1$ either confirms the receipt of the role switch signal (a $0$ heard before any $1$'s in a block), or the party already received the switch signal earlier and is already in $\speaker$ mode; either way, the $\passer$ is free to switch to $\listener$ mode in the next block since the other party will be in $\speaker$ mode.
    % (since they only send $0$ while in $\passer$ mode, the other party cannot transition out of $\speaker$ mode).
\end{itemize}

In this way, the roles of the $\speaker$ and $\listener$ have now switched and the protocol is in an entirely ``reset'' state with one more bit of the noiseless transcript $\pi_0$ having been conveyed.

To understand why this protocol is resilient to $\frac12-\epsilon$ erasures, we use the following fact: There are at least $\approx n$ blocks with $<\frac12-\epsilon$ erasures, and in each such block, there are at least a constant, say 2, pairs of consecutive messages that are unerased. In each such pair of messages, the protocol will make \emph{progress} via one party hearing the other and successfully confirming receipt of the message. (Formally, these two pairs of unerased consecutive messages are enough to ensure that at least one party completes the goal for that mode and advances modes at the end of the block.) 

For a formal description and analysis of this protocol, we refer the reader to Section~\ref{sec:erasure}.

==> intro/overview-old.tex <==
\subsection{Technical Overview}\label{sec:overview}

\subsubsection{Error Resilient Communication Over Binary Erasure Channels}

We first remark that $\frac12$ is the maximal possible erasure resilience of a two-party interactive protocol over \emph{any} alphabet: the adversary can simply erase all messages of the party that speaks less. 

Previous attempts to construct maximally erasure resilient interactive protocols over the binary alphabet did so by starting with such a protocol over a larger alphabet and then replacing each character with a binary error correcting code. For instance, in~\cite{EfremenkoGH16}, they constructed a protocol resilient to $\frac12$ erasures over an alphabet of size 4, then replaced the alphabet with the four strings $(000)^*, (110)^*, (101)^*, (011)^*$ that have relative distance $\frac23$. This resulted in an binary protocol resilient to $\frac12 \cdot \frac23 = \frac13$ erasures. Unfortunately, $\frac13$ is also the maximal erasure resilience attainable with this approach, as $\frac12$ is the maximal erasure resilience of a protocol over any alphabet and $>2$ binary codewords necessarily have relative distance $\le \frac23$.

In our paper, we deviate from this strategy of substituting binary codewords for a larger alphabet. Instead, we leverage a key property of communication over erasure channels, which is that \emph{communication can be delayed but not wrong}. That is, Alice and Bob simulate a noiseless protocol $\pi_0$ by sending the next bit of $\pi_0$ \emph{until they are sure} that the other party has received their message. Then, they simply have to let the other party know that it is their turn to talk. 

The challenge is to do this using only a binary alphabet. Intuitively, a speaker has three things to communicate: the bit $0$, the bit $1$, and switching speakers. Communicating these with three binary codewords doesn't work, as discussed above.

Instead, we observe that we can let the bits $0$ and $1$ mean \emph{more than two things} if we combine them with timing cues, such that $0$ and $1$ mean different things when heard at different parts of the protocol. More specifically, we partition the protocol into \emph{blocks} of many rounds. In each block, the first bit that the listener receives tells them whether the speaker is trying to send a bit or switch speakers. That is, if the first bit heard within the block is a $1$, they know that the speaker is trying to communicate a bit, and if the first bit heard is a $0$, then they know to become the speaker starting next block. In response to each message from the speaker, the listener sends $1$ if they received the message and $0$ if it was erased. On the other hand, if the speaker wants to send a bit $b$, they send $1$'s until they receive signal that the listener has heard it, at which point they send $b$ for the rest of the block. If the speaker wants to switch speakers, they send $0$'s the entire block.

In the case that the first bit heard by the listener is a $1$, ideally the rest of the bits heard within the block would tell them what the speaker's message was. However, this is not necessarily the case: if the listener only receives $1$'s within a block, the adversary may have corrupted enough of the block so that the listener didn't receive the bit the speaker wanted to communicate, or the speaker never got signal that the listened heard a $1$ and thus never got around to sending $b$. In these cases, the speaker's message is ambiguous. Fortunately though, there is one block in which the listener must've received both bits the speaker wanted to send: the last block prior to receiving a speaker switch signal in which not all messages from the sender were erased. This is the case since the speaker sends all $0$'s only when they know for sure that the listener received both bits. Thus, when the listener receives the signal to switch speakers, they can correctly determine the speaker's next bit in $\pi_0$ and begin sending their own next bit in $\pi_0$. In this way, Alice and Bob simulate $\pi_0$ bit by bit.

For a formal description and analysis of this protocol, we refer the reader to Section~\ref{sec:erasure}.


\subsubsection{Error Resilient Communication Over Binary Bit Flip Channels}

We begin with the following (flawed) approach, which achieves an error resilience of $\frac18$: Alice sends $\ECC(x)$, and Bob sends $\ECC(y)$. Since $\ECC$ has a minimal relative distance of at most $\frac12$, the adversary can simply flip $\frac14$ of the party that speaks less so that the other party cannot distinguish between two inputs.

Recall that the maximal error resilience of any binary two-party protocol is $\frac13$ of either party's communication. The above flawed protocol only had error resilience of $\frac14$ of either party's communication. In order to increase this to $\frac13$, we introduce a new \emph{question-answer} approach: in each round of interaction, a party asks a question (encoded with an $\ECC$) about the other party's input, and the other party responds with one of \emph{four} answers that can have relative distance $\frac23$. Now, if the adversary simply corrupts the answers, she'd have to corrupt $\frac12 \cdot \frac23 = \frac13$ of the answering party's rounds.

While this achieves $\frac13$ resilience for the answering party's communication, the asking party's communication is still only $\frac14$-error resilient as they are sending an error correcting code. In order to attain $\frac13$ error resilience for \emph{both} parties, both parties will need to \emph{simultaneously ask and answer a question} each round.

More specifically, Alice and Bob each keep track of a guess $\hat{y}$ or $\hat{x}$ respectively for the other party's input. At first, $\hat{y} = \hat{x} = \emptyset$. Each round, Alice (resp. Bob) asks the other party for one of four operations to do to $\hat{y}$ (resp. $\hat{x}$): append $0$ ($0$), append $1$ ($1$), delete the last bit ($\rewind$), or ``bingo -- you got it right!'' ($\bullet$). They also keep track of counters $c_A$ and $c_B$ respectively that indicate how many times they've received the ``bingo'' message from the other party for their current guess $\hat{y}$ or $\hat{x}$: receiving $\bullet$ increases $c_A$ (resp. $c_B$) by $1$, and receiving $\rewind$ decreases $c_A$ (resp. $c_B$) by $1$. 

To answer a question, a party responds with the question that was just asked, followed by one of the four operations $0,1,\rewind,\bullet$. That is, each of Alice's messages is of the form $(\hat{y}, x^*, \delta^*)$, where $y^*$ is the question she just heard from Bob and $\delta^* \in \{ 0,1,\rewind,\bullet \}$. Likewise Bob's messages are of the form $\ECC(\hat{x}, y^*, \delta^*)$. Alice only performs an update on $\hat{y}$ if Bob's message satisfies $y^* = \hat{y}$.

The $\ECC$ we use has relative distance $\ge \frac12$ between all pairs of codewords, and has relative distance $\frac23$ between codewords of the form $\ECC(x', y', \delta_0)$ and $\ECC(x', y', \delta_1)$ where $\delta_0 \not= \delta_1$. The idea is that if the adversary only corrupts Bob's answer, it will require $\frac13$ corruptions of Bob's communication for Alice to output the wrong $y$.

However, it seems as if we have lost the advantage we gained earlier: the adversary can corrupt both Bob's answer \emph{and question} every other round so that Alice receives $\ECC(x', \hat{y}, \delta')$, where $x' \not= \hat{x}$ and $\delta' \not= \delta^*$. Then, every other round, Alice performs an incorrect update on $\hat{y}$ and $c_A$, so that over time she gets no closer to learning $y$. Furthermore, this attack only requires corrupting $\frac12$ of Bob's message every other round, for a total of $\frac14$ of his total communication.

Let us analyze this situation more closely. We count progress as number of good updates (getting closer to the other party's input) minus the number of bad updates (getting further from the other party's input). What happens is that the adversary can corrupt $\frac12$ of Bob's message to get $-1$ progress for Alice and $0$ progresss for Bob (Alice answers the wrong question for Bob so that he performs no update), from an original progress count of $(+1, +1)$ had no corruptions occurred. So, when the adversary corrupts every other of Bob's messages, Alice's progress count remains $0$, but Bob's increases at a steady rate! If there were a way to balance this, so that when Bob has made lots of progress it becomes harder to cause negative progress for Alice, perhaps we could achieve our goal of $\frac13$ error resilience for each party.

To do this, we make the following change to the way Alice and Bob make updates to their current guesses $\hat{y}$ and $\hat{x}$: they only update $\hat{y}$ (resp. $\hat{x}$) with probability $1$ if the question they just received is equal to their input, otherwise they update $\hat{y}$ (resp. $\hat{x}$) with probability $0.5$. This way, when Bob has made lots of progress so that $\hat{x} = x$, if the adversary corrupts Bob's message to be $\ECC(x' \not= x, \hat{y}, \delta')$, Alice only updates $\hat{y}$ with probability $0.5$ --- $-0.5$ progress instead of $-1$! Now, when Bob has made lots of progress, the adversary has to corrupt two out of every three of Bob's messages in order for Alice to remain at $0$ progress, bringing us up to a $\frac13$ corruption rate.

This change in update probability introduces a new situation, which is that when both Alice and Bob have made little progress, the adversary can corrupt Bob's message to be $\ECC(x \not= \hat{x}, \hat{y}, \delta')$ so that Alice performs a bad update with probability $1$, i.e. $(-1, 0)$ progress, from an original $(+0.5, +0.5)$ progress without corruption. Then, if the adversary corrupts one message every two rounds of interaction, the total progress between Alice and Bob remains $0$! To remedy this, we have Alice and Bob perform an additional update with probability $0.5$ when they see that the answer is of the form $(y', \bullet)$ (resp. $(x', \bullet)$) with $|y'| = n$ (resp. $|x'| = n$). Now, when Bob receives Alice's response $\ECC(\hat{y}, x, \bullet)$ to his corrupted question, he performs a $+0.5$ update, so that the total effect of the adversary's corruption to Bob's message is $(-1, +0.5)$, i.e. a $-0.5$ bad collective bad update.

So far, we've only specified Alice and Bob's behavior when they receive a codeword. Since an adversary can corrupt messages in any manner, we must also specify Alice and Bob's behavior when they receive \emph{any} sequence of bits, not just valid codewords. To do this, we say that when Alice receives a message from Bob, she ``rounds'' to the nearest full codeword and does the corresponding update depending on the distance to the codeword. 

For a formal description of the protocol and a detailed analysis, we refer the reader to Section~\ref{sec:toggle}.

% main points:
% - 1/8 is attained by ECC, ECC - bad because the adversary can corrupt 1/4 of one person
% - we instead develop question-answer paradigm - where answer is one of <=4 so answers can be 2/3 apart
% - but need to answer while also asking - say send ECC(hat{y}, x*, delta*)
% - issue is there are /many/ questions, so that distance between answers has seemingly now gone down to 1/2 again! 
% - what happens is that you can corrupt 1/2 and get (-1,0) damage, from an original (+1,+1) progress. issue is one party can be at 0 progress while the other is at + a lot -- is there a way to balance this out so that if the other party has lots of progress, then its harder to make damage to the first party? eg (-0.5, 0) from (+1, +1)
% - yes! when the other party sends hat{x} = x, then alice should update +1. if not then alice updates +0.5. 
% - new situation: the adversary can now corrupt a (+0.5, +0.5) to a (-1, 0) -- so introduce second update \bullet to correct to (-1, 0.5)



==> intro/related.tex <==
\subsection{Related Work}

\paragraph{Interactive Coding.}
Non-adaptive interactive coding has studied starting with the seminal works of Schulman~\cite{Schulman92,Schulman93,Schulman96} and continuing in a prolific sequence of followup works, including~\cite{BravermanR11,Braverman12,BrakerskiK12,BrakerskiN13,Haeupler14,BravermanE14,GellesHKRW16, GellesH17,EfremenkoGH16,GhaffariH13,EfremenkoKS20b}. We note that there are many other works studying variations upon this original interactive coding setup, including adaptive and multi-party schemes. We refer the reader to an excellent survey by Gelles~\cite{Gelles-survey} for an extensive list of related work. 
    
\paragraph{Error Correcting Codes with Feedback.}
Outside of interactive coding, optimal error resilience of an interactive protocol has been studied in the context of \emph{error correcting codes with feedback},\footnote{We remark that this notion of \emph{feedback} is different than the aforementioned notion of channels with noiseless feedback. In the previous notion of channels with feedback, } first introduced by~\cite{Berlekamp64}. In an error correcting code with feedback, Alice's goal is to communicate a message to Bob in an error resilient way. For every message she sends, Bob sends her uncorrupted feedback that is not counted towards the adversary's budget.

\cite{Berlekamp68,Zigangirov76,SpencerW92} showed that in the bit flip error model, the maximal error resilience of an error correcting code with feedback over a binary alphabet is $\frac13$. In other words, in any binary protocol where Alice is trying to convey some information to Bob, as long as the adversary corrupts fewer than $\frac13$ of Alice's messages, Bob learns Alice's input successfully. Assuming that Alice and Bob speak equal amounts, this translates to a binary protocol resilient to $\frac16$ corruptions --- as long as all corruptions are to Alice's messages. 

Our $\frac16$ protocol can be seen as a strengthening of optimal error correcting codes with feedback: Now, \emph{both} Alice and Bob can learn the other's input, where the protocol is resilient to $\frac13$ corruptions to either party or more generally to any corruption pattern totaling to less than $\frac16$ of the total communication. In particular, we show that it is possible for both parties to \emph{simultaneously} communicate information about their input and give feedback. 



==> toggle/1.6-orig/analysis.tex <==
\subsection{Analysis}

We begin by showing that there is at most one triple $(x', y', \delta')$ for which $p$ and $q$ are positive, so that $(x_B, y_B, \delta_B)$ is uniquely defined for each message $m$ Alice receives. 

\begin{lemma} \label{onep}
    The following holds for $p$ and $q$ defined in Protocol~\ref{prot:1/6}:
    \begin{enumerate}[label={(\arabic*)}]
        \item For any message $m$ and triple $(x', y', \delta')$, it holds that $p(x', y', \delta') > 0 \Longleftrightarrow q(x', y', \delta') > 0$.
        \item For any message $m$, there is at most one triple $(x', y', \delta')$ for which $p(x', y', \delta'), q(x', y', \delta') > 0$.
    \end{enumerate}
\end{lemma}

\begin{proof}
    We prove the two parts:
    
    \begin{enumerate}[label={(\arabic*)}]
    \item 
        Fix any $m$ and $(x', y', \delta')$. If $x' = x$, then $b(x', y') = 1$, so then $p(x', y', \delta') = 1 - 3d(x', y', \delta') = q(x', y', \delta')$. If $x' \not= x$, then $b(x', y') = 0$, and $p(x', y', \delta') = \frac12 - 3d(x', y', \delta')$ and $q(x', y', \delta') = 1 - 6 d(x', y', \delta')$, or $p(x', y', \delta') = \frac12 q(x', y', \delta')$. In either case, $p(x', y', \delta') > 0 \Longleftrightarrow q(x', y', \delta') > 0$.
    \item 
        Fix any message $m$. It suffices to show that there is at most one triple $(x', y', \delta')$ for which $p(x', y', \delta') > 0$, as the sign of $p(x', y', \delta')$ and $q(x', y', \delta')$ is the same. To do this, we will show that for any two triples $(x', y', \delta') \not= (x'', y'', \delta'')$, 
        \[
            \frac{2 + b(x', y') + b(x'', y'')}{6} \le \Delta(\ECC(x', y', \delta'), \ECC(x'', y'', \delta'')), \numberthis \label{eqn:onep-todo}
        \]
        as this implies that 
        \begin{align*}
            \frac{2 + b(x', y') + b(x'', y'')}{6} 
            &\le \Delta(\ECC(x', y', \delta'), \ECC(x'', y'', \delta'')) \\
            &\le \Delta(m, \ECC(x', y', \delta')) + \Delta(m, \ECC(x'', y'', \delta'')) \\
            \implies p(x', y', \delta') &+ p(x'', y'', \delta'') \le 0,
        \end{align*}
        meaning that at least one of $p(x', y', \delta')$ and $p(x'', y'', \delta'')$ must not be positive.
        
        We show Equation~\eqref{eqn:onep-todo} by cases on the values of $b(x', y')$ and $b(x'', y'')$. W.l.o.g. we assume $b(x', y') \le b(x'', y'')$.
        
        \begin{caseof}
            \case{$b(x', y') = b(x'', y'') = 1$.}{
                This implies that $x' = x = x''$ and $y' = \hat{y} = y''$, so since $(x', y', \delta') \not= (x'', y'', \delta'')$, it must be that $\delta' \not= \delta''$. Then, Equation~\eqref{eqn:onep-todo} is implied by
                \[
                    \frac23 \le \Delta(\ECC(x, \hat{y}, \delta'), \ECC(x, \hat{y}, \delta'')) = \frac23.
                \]
            }
            \case{$b(x', y') = 0$ and no restrictions on $b(x'', y'')$.}{
                Note that in all cases where $(x', y', \delta') \not= (x'', y'', \delta'')$, it holds that $\Delta(\ECC(x, \hat{y}, \delta'), \ECC(x, \hat{y}, \delta'')) \ge \frac12$. Furthermore, $b(x', y') + b(x'', y'') = b(x'', y'') \le 1$. Then, Equation~\eqref{eqn:onep-todo} is implied by
                \[
                    \frac{2 + b(x', y') + b(x'', y'')}{6} 
                    \le \frac12 
                    \le \Delta(\ECC(x, \hat{y}, \delta'), \ECC(x, \hat{y}, \delta'')).
                \]
            }
        \end{caseof}
    \end{enumerate}
\end{proof}

We now state our main error resilience theorem.

\begin{theorem} \label{thm:1/6}
    Assuming that every message received by Alice and Bob is a codeword, then Protocol~\ref{prot:1/6} has an error resilience of $\frac16 - \epsilon$ with probability $1 - 2\exp \left( \frac{-\epsilon N}{100} \right)$.
\end{theorem}

To prove Theorem~\ref{thm:1/6}, we analyze the effects of corruption on the \emph{good} and \emph{bad updates} Alice/Bob make. We begin by defining good and bad updates.

After receiving a message from Bob, Alice performs an update (with some probability) to her values of $c_A$ and $\hat{y}$. We say that an update is \emph{good} if $\hat{y} = y$ and the update was $c_A \gets c_A + 1$, or if $\hat{y} \not= y$ and the update was either $c_A \gets c_A - 1$ if $c_A > 0$ or $\hat{y} \gets \hat{y} + \sign(y - \hat{y})$ if $c_A = 0$. Otherwise, an update is \emph{bad} if $\hat{y} = y$ and the update was $c_A \gets c_A - 1$ or if $\hat{y} \not= y$ and the update was either $c_A \gets c_A + 1$ or $\hat{y} \gets \hat{y} - \sign(y - \hat{y})$. We similarly define good and bad updates for Bob.

For each $t \in [0, \dots, T]$, we define the following potential functions:
\begin{itemize}
    \item $\psi^A_t$ is defined to be the total number of good updates minus the number of bad updates Alice has done in response to messages $0, \dots, t$.
    \item $\psi^B_t$ is defined to be the total number of good updates minus the number of bad updates Bob has done in response to messages $0, \dots, t$.
\end{itemize}
For instance, $\bbE[\psi^A_0] = 0.5$ and $\psi^B_0 = 0$. 

\begin{lemma} \label{lemma:N}
    After message $t$, $\psi_t^A \ge N$ if and only if Alice's value of $\hat{y}$ is equal to $y$, and $\psi^B_t \ge N$ if and only if Bob's value of $\hat{x}$ is equal to $x$.
    
    In particular, at the end of the protocol, Alice outputs $\hat{y} = y$ iff $\psi^A_T \ge N$, and Bob outputs $\hat{x}$ iff $\psi^B_T \ge N$.
\end{lemma}

\begin{proof}
    We prove this for Alice, as the statement for Bob follows identically. We keep track of the number of good updates Alice must do to have $\hat{y} = y$. Note that any good update decreases this number by $1$, and any bad update increases this number by $1$. Furthermore, before the protocol has started, the number of good updates Alice needs to do before $\hat{y} = y$ is $N$. Thus, $\hat{y} = y$ if and only if the number of good updates minus the number of bad updates is at least $N$.
\end{proof}

For Alice, we group each consecutive pair of Alice-to-Bob and Bob-to-Alice messages (i.e. messages $2k-1$ and $2k$), and for Bob, we group each consecutive pair of Bob-to-Alice and Alice-to-Bob messages (i.e. messages $2k-2$ and $2k-1$), starting with the unsent message $0$ which we recall is understood to be $\ECC(0,0,+1)$. We define the following potential function for each $k \in [1, T/2]$: 
\begin{itemize}
    \item $\Psi^A_k = \psi^A_{2k} + \min \{ \psi^B_{2k} + \min \{ \rho^B_{2k+1}, 0.5 \}, N \}$
    \item $\Psi^B_k = \psi^B_{2k-1} + \min \{ \psi^A_{2k-1} + \min \{ \rho^A_{2k}, 0.5 \}, N \}$,
\end{itemize}
where $\rho^A_t$ and $\rho^B_t$ are defined as follows:
\begin{itemize}
    \item For even $t$, $\rho^A_t$ is the expected number of good updates minus the number of bad updates that Alice will do in response to message $t$, given messages $1,\dots,t-1$, if message $t$ from Bob is uncorrupted.
    \item For odd $t$, $\rho^B_t$ is the expected number of good updates minus the number of bad updates that Bob will do in response to message $t$, given messages $1,\dots,t-1$, if message $t$ from Alice is uncorrupted. For instance, $\bbE[\rho^B_1] = 0.5$.\rnote{this is only true if we switch to rewind if error ; otherwise alice could possibly have updated $\hat{y}$ to be $1 = y$.}
\end{itemize} 

\begin{lemma} \label{lemma:0.5-3alpha}
    If an $\alpha_{2k-1}$ fraction of message $2k-1$ and an $\alpha_{2k}$ fraction of message $2k$ is corrupted, then 
    \[
        \bbE [\Psi^A_k - \Psi^A_{k-1}] \ge 1 - 3\alpha_{2k-1} - 3\alpha_{2k}. \numberthis \label{eqn:alice-0.5-3alpha}
    \]
    If an $\alpha_{2k-2}$ fraction of message $2k-2$ and an $\alpha_{2k-1}$ fraction of message $2k-1$ is corrupted, then
    \[
        \bbE [\Psi^B_k - \Psi^B_{k-1}] \ge 1 - 3\alpha_{2k-2} - 3\alpha_{2k-1}. \numberthis \label{eqn:bob-0.5-3alpha}
    \]
\end{lemma}

\begin{proof}
    We only prove Inequality~\eqref{eqn:alice-0.5-3alpha}, as the proof for Inequality~\eqref{eqn:bob-0.5-3alpha} is identical.
    
    Define $\Psi_k$ to be $\psi^A_{2k} + \rho^A_{2k} + \min \{ \psi^B_{2k-1}, N \}$. We will first determine the value of $\bbE[ \Psi^A_k - \Psi_k ]$.
    
    \begin{claim}
        If $\psi^B_{2k-1} < N$, then 
        \[
            \bbE [ \Psi^A_k - \Psi_k ] \ge 0.5 - 3\alpha_{2k}.
        \]
        If $\psi^B_{2k-1} \ge N$, then
        \[
            \bbE [ \Psi^A - \Psi_k ] \ge -3\alpha_{2k}.
        \]
    \end{claim}
    
    \begin{proof}
    
        Define $U_{2k}$ to be the good minus bad update Alice makes in response to message $2k$. Let Bob's intended message for message $2k$ be $\ECC(x_{2k},y_{2k},\delta_{2k})$. Alice will calculate $p_{2k}, q_{2k}, \ECC(x'_{2k},y'_{2k},\delta'_{2k})$ as in Lemma~\ref{onep}. If they do not exist, let them be $0,0,\ECC(x_{2k},y_{2k},\delta_{2k})$. Since $p_{2k}=q_{2k}=0$, it does not matter that Alice cannot actually compute these values.
        
        \begin{caseof}
            \case{$\psi^B_{2k-1} < N$: then $\bbE[\Psi^A_k - \Psi_k] \ge 0.5 - 3\alpha_{2k}$}{
                We have 
                \begin{align*}
                    \bbE[\Psi^A_k - \Psi_k] &= \psi^A_{2k} + \min \{ \psi^B_{2k} + \min \{ \rho^B_{2k+1}, 0.5 \}, N \} - \psi^A_{2k-1} - \rho^A_{2k} - \min \{ \psi^B_{2k-1}, N \} \\
                    &= \bbE [U_{2k}-\rho^A_{2k}+\min \{ \rho^B_{2k+1}, 0.5 \}]
                \end{align*}
                because $\psi^B_{2k-1}=\psi^B_{2k}\leq N-1$ and $\rho^B_{2k+1}\leq 1$. 
                
                By Lemma~\ref{lemma:N}, Bob does not know $x$, so $x_{2k}\neq x$. 
                
                \begin{subcaseof}
    
                \subcase {$(x_{2k},y_{2k},\delta_{2k}) = (x'_{2k},y'_{2k},\delta'_{2k})$ and ($y_{2k}=\hat{y}$ or $\delta_{2k}=0$).}
                { If Alice updates, she performs a good update, and since $x'_{2k} \neq x$, we have $\rho^A_{2k}=0.5$. She updates with probability $p_{2k}\geq 0.5-3\alpha_{2k}$, since the distance to the original message is at most the corruption. Her probability is calculated as such because we are in the case where $x'_{2k}\neq x$. Therefore, $\bbE [U_{2k}]\geq 0.5-3\alpha_{2k}$. If Alice decides to answer with $\ECC(x,\hat{y}, 0)$, so $\rho^B_{2k+1}$ will be either $0.5$ or $1$, and similarly if she answers with $\ECC(x_{2k},\hat{y}, \delta)$ for the correct $\delta$, $\rho^B_{2k+1}$ will be either $0.5$ or $1$. In either case, $\min \{ \rho^B_{2k+1}, 0.5 \} =0.5$. Then 
                \[
                    \bbE[\Psi^A_k - \Psi_k] = \bbE [U_{2k}-\rho^A_{2k}+\min \{ \rho^B_{2k+1}, 0.5 \}] \geq 0.5-3\alpha_{2k}-0.5+0.5=0.5-3\alpha_{2k}.
                \]
                }
                \subcase {$(x_{2k},y_{2k},\delta_{2k}) = (x'_{2k},y'_{2k},\delta'_{2k})$ and ($y_{2k}\neq \hat{y}$ and $\delta_{2k}\neq 0$).}
                { Alice will never update, and is not expected to in response to the original message. As such, $U_{2k}=0$ and $\rho^A_{2k}=0$. If Alice decides to answer with $\ECC(x,\hat{y}, 0)$, so $\rho^B_{2k+1}$ will be either $0.5$ or $1$, and similarly if she answers with $\ECC(x_{2k},\hat{y}, \delta)$ for the correct $\delta$, $\rho^B_{2k+1}$ will be either $0.5$ or $1$. In either case, $\min \{ \rho^B_{2k+1}, 0.5 \} =0.5$. Then 
                \[
                    \bbE[\Psi^A_k - \Psi_k] = \bbE [U_{2k}-\rho^A_{2k}+\min \{ \rho^B_{2k+1}, 0.5 \}] \geq 0-0+0.5\geq 0.5-3\alpha_{2k}.
                \]
                }
                \subcase {$(x_{2k},y_{2k},\delta_{2k}) \neq (x'_{2k},y'_{2k},\delta'_{2k})$ and $x'_{2k}=x$.}
                { Notice that $\rho^A_{2k}\leq 0.5$, since $x_{2k}\neq x$. If Alice updates, she performs a bad update. Let $d_{2k}$ be the distance to $\ECC(x'_{2k},y'_{2k},\delta'_{2k})$. She updates with probability $p_{2k}= 1-3d_{2k}$ or 0 depending on $y'_{2k}$ and $\delta'_{2k}$. Her probability is calculated as such because we are in the case where $x'_{2k}= x$. Notice that $d\geq \frac12-\alpha_{2k}$ since $\frac12$ is the $\ECC$ distance, and so $p_{2k}\leq 3\alpha_{2k}-0.5$. Therefore, $\bbE [U_{2k}]\geq 0.5-3\alpha_{2k}$ since the update is bad, and $\bbE [U_{2k}-\rho^A_{2k}]\geq -3\alpha_{2k}$. Since $x'_{2k}=x$, Alice will always answer with $\ECC(x,\hat{y}, 0)$, so $\rho^B_{2k+1}$ will be either $0.5$ or $1$, so $\min \{ \rho^B_{2k+1}, 0.5 \} =0.5$. Then 
                \[
                    \bbE[\Psi^A_k - \Psi_k] = \bbE [U_{2k}-\rho^A_{2k}+\min \{ \rho^B_{2k+1}, 0.5 \}] \geq -3\alpha_{2k}+0.5=0.5-3\alpha_{2k}.
                \]
                }
                \subcase {$(x_{2k},y_{2k},\delta_{2k}) \neq (x'_{2k},y'_{2k},\delta'_{2k})$ and $x'_{2k}\neq x$.}
                { Notice that $\rho^A_{2k}\leq 0.5$, since $x_{2k}\neq x$. If Alice updates, she performs a bad update. Let $d_{2k}$ be the distance to $\ECC(x'_{2k},y'_{2k},\delta'_{2k})$. She updates with probability $p_{2k}= 0.5-3d_{2k}$ or 0 depending on $y'_{2k}$ and $\delta'_{2k}$. Her probability is calculated as such because we are in the case where $x'_{2k}\neq x$. Notice that $d\geq \frac12-\alpha_{2k}$ since $\frac12$ is the $\ECC$ distance, and so $p_{2k}\leq 3\alpha_{2k}-1$. Therefore, $\bbE [U_{2k}]\geq 1-3\alpha_{2k}$ since the update is bad, and $\bbE [U_{2k}-\rho^A_{2k}]\geq 0.5-3\alpha_{2k}$. It is always the case that $\min \{ \rho^B_{2k+1}, 0.5 \} > 0$. Then 
                \[
                    \bbE[\Psi^A_k - \Psi_k] = \bbE [U_{2k}-\rho^A_{2k}+\min \{ \rho^B_{2k+1}, 0.5 \}] \geq 0.5-3\alpha_{2k}.
                \]
                }
                \end{subcaseof}
            }
            
            \case{$\psi^B_{2k-1} \ge N$: then $\bbE[\Psi^A_k - \Psi_k] \ge - 3\alpha_{2k}$}{
                We have 
                \begin{align*}
                    \bbE[\Psi^A_k - \Psi_k] &= \psi^A_{2k} + \min \{ \psi^B_{2k} + \min \{ \rho^B_{2k+1}, 0.5 \}, N \} - \psi^A_{2k-1} - \min \{ \psi^B_{2k-1}, N \} \\
                    &= \bbE [U_{2k}-\rho^A_{2k}]
                \end{align*}
                because $\psi^B_{2k-1}=\psi^B_{2k}\leq N-1$ and $\rho^B_{2k+1}\leq 1$. 
                
                By Lemma~\ref{lemma:N}, Bob does knows $x$, so $x_{2k} = x$. 
                
                \begin{subcaseof}
                \subcase {$(x_{2k},y_{2k},\delta_{2k}) = (x'_{2k},y'_{2k},\delta'_{2k})$ and ($y_{2k}=\hat{y}$ or $\delta_{2k}=0$).}
                { If Alice updates, she performs a good update, and since $x'_{2k} = x$, we have $\rho^A_{2k}=1$. She updates with probability $p_{2k}\geq 1-3\alpha_{2k}$, since the distance to the original message is at most the corruption. Her probability is calculated as such because we are in the case where $x'_{2k} = x$. Therefore, $\bbE [U_{2k}]\geq 0.5-3\alpha_{2k}$. Then 
                \[
                    \bbE[\Psi^A_k - \Psi_k] = \bbE [U_{2k}-\rho^A_{2k}] \geq 1-3\alpha_{2k}-1=-3\alpha_{2k}.
                \]
                }
                \subcase {$(x_{2k},y_{2k},\delta_{2k}) = (x'_{2k},y'_{2k},\delta'_{2k})$ and ($y_{2k}\neq \hat{y}$ and $\delta_{2k}\neq 0$).}
                { Alice will never update, and is not expected to in response to the original message. As such, $U_{2k}=0$ and $\rho^A_{2k}=0$. Then 
                \[
                    \bbE[\Psi^A_k - \Psi_k] = \bbE [U_{2k}-\rho^A_{2k}] \geq 0-0+\geq -3\alpha_{2k}.
                \]
                }
                \subcase {$(x_{2k},y_{2k},\delta_{2k}) \neq (x'_{2k},y'_{2k},\delta'_{2k})$ and $x'_{2k}=x$.}
                { Notice that $\rho^A_{2k}\leq 1$, since $x_{2k} = x$. If Alice updates, she performs a bad update. Let $d_{2k}$ be the distance to $\ECC(x'_{2k},y'_{2k},\delta'_{2k})$. She updates with probability $p_{2k}= 1-3d_{2k}$ or 0 depending on $y'_{2k}$ and $\delta'_{2k}$. Her probability is calculated as such because we are in the case where $x'_{2k}= x$. Notice that $d\geq \frac23-\alpha_{2k}$ since $\frac23$ is the $\ECC$ distance, and so $p_{2k}\leq 3\alpha_{2k}-1$. Therefore, $\bbE [U_{2k}]\geq 1-3\alpha_{2k}$ since the update is bad. Then 
                \[
                    \bbE[\Psi^A_k - \Psi_k] = \bbE [U_{2k}-\rho^A_{2k}] \geq -3\alpha_{2k}.
                \]
                }
                \subcase {$(x_{2k},y_{2k},\delta_{2k}) \neq (x'_{2k},y'_{2k},\delta'_{2k})$ and $x'_{2k}\neq x$.}
                { Notice that $\rho^A_{2k}\leq 1$, since $x_{2k} = x$. If Alice updates, she performs a bad update. Let $d_{2k}$ be the distance to $\ECC(x'_{2k},y'_{2k},\delta'_{2k})$. She updates with probability $p_{2k}= 0.5-3d_{2k}$ or 0 depending on $y'_{2k}$ and $\delta'_{2k}$. Her probability is calculated as such because we are in the case where $x'_{2k}\neq x$. Notice that $d\geq \frac12-\alpha_{2k}$ since $\frac12$ is the $\ECC$ distance, and so $p_{2k}\leq 3\alpha_{2k}-1$. Therefore, $\bbE [U_{2k}]\geq 1-3\alpha_{2k}$ since the update is bad. Then 
                \[
                    \bbE[\Psi^A_k - \Psi_k] = \bbE [U_{2k}-\rho^A_{2k}] \geq -3\alpha_{2k}.
                \]
                }
                \end{subcaseof}
            }
        
        \end{caseof}
    
    \end{proof}
    
    We return to calculating $\bbE [ \Psi^A_k - \Psi^A_{k-1} ]$. Define $U_{2k-1}$ to be the good minus bad update Bob makes in response to message $2k-1$. Let Alice's intended message for message $2k-1$ be $\ECC(x_{2k-1},y_{2k-1},\delta_{2k-1})$. Bob will calculate $p_{2k-1}, q_{2k-1}, \ECC(x'_{2k-1},y'_{2k-1},\delta'_{2k-1})$ as in Lemma~\ref{onep}. If they do not exist, let them be $0,0,\ECC(x_{2k-1},y_{2k-1},\delta_{2k-1})$. Since $p_{2k-1}=q_{2k-1}=0$, it does not matter that Bob cannot actually compute these values.
    We have 
    \begin{align*}
        \bbE[\Psi_k - \Psi^A_{k-1}] &= \bbE [\psi^A_{2k-1} + \rho^A_{2k} + \min \{ \psi^B_{2k-1}, N \} - \psi^A_{2k-2} - \min \{ \psi^B_{2k-2} + \min \{ \rho^B_{2k-1}, 0.5 \}, N \}] \\
        &= \bbE [\min \{ \psi^B_{2k-1}, N \} - \min \{ \psi^B_{2k-2} + \min \{ \rho^B_{2k-1}, 0.5 \}, N \} + \rho^A_{2k}]
    \end{align*}
    because Alice neither updates nor is expected to in response to message $2k-1$ which she sends. 
        
    \begin{caseof}
    \case{$\psi^B_{2k-2} < N$:} {
        We have 
        \begin{align*}
            \bbE[\Psi_k - \Psi^A_{k-1}] &= \bbE [\min \{ \psi^B_{2k-1}, N \} - \min \{ \psi^B_{2k-2} + \min \{ \rho^B_{2k-1}, 0.5 \}, N \}] \\
            &= \bbE [\min \{ \psi^B_{2k-1}, N \}- \psi^B_{2k-2} - \min \{ \rho^B_{2k-1}, 0.5 \}+ \rho^A_{2k}] \\
            &= \bbE [\psi^B_{2k-1}- \psi^B_{2k-2} - \min \{ \rho^B_{2k-1}, 0.5 \}+ \rho^A_{2k}] \\
            &= \bbE [U_{2k-1} - \min \{ \rho^B_{2k-1}, 0.5 \}+ \rho^A_{2k}]
        \end{align*}
        because $\psi^B_{2k-1}\leq N-1$, and adjacent values can differ by at most 1, so $\psi^B_{2k-1}\leq N$.
    
        By Lemma~\ref{lemma:N}, Bob does not know $x$ after message $2k-2$, so $x_{2k-2}\neq x$. 
        \begin{subcaseof}
        \subcase{$(x_{2k-1},y_{2k-1},\delta_{2k-1}) = (x'_{2k-1},y'_{2k-1},\delta'_{2k-1})$ and ($y_{2k-1}=y$ and $x_{2k-1}=\hat{x}$).}
        { If Bob updates, he performs a good update, and since $y'_{2k-1} = y$ and $x_{2k-1}=\hat{x}$, we have $\rho^B_{2k-1}=1$. He updates with probability $p_{2k-1}\geq 1-3\alpha_{2k-1}$, since the distance to the original message is at most the corruption. His probability is calculated as such because we are in the case where $y'_{2k-1} = y$ and $x_{2k-1}=\hat{x}$. Therefore, $\bbE [U_{2k-1}]\geq 1-3\alpha_{2k-1}$, and so $\bbE [U_{2k-1} - \min \{ \rho^B_{2k-1}, 0.5 \}]\geq 1-3\alpha_{2k-1}-0.5=0.5-3\alpha_{2k-1}$.
        
        Now, we evaluate $\bbE [\rho^A_{2k}+\Psi^A_k - \Psi_k]$. Regardless of what message Bob sends, $\rho^A_{2k} \geq 0.5$, and from the previous calculation we know $\bbE [\Psi^A_k - \Psi_k] \geq -3\alpha_{2k-1}$, so we have 
        \[
            \bbE[\Psi^A_k - \Psi^A_{k-1}] = \bbE [\Psi^A_k - \Psi_k + U_{2k-1} - \min \{ \rho^B_{2k-1}, 0.5 \}+ \rho^A_{2k}] \geq -3\alpha_{2k}+0.5-3\alpha_{2k-1}+0.5=1-3\alpha_{2k-1}-3\alpha_{2k}.
        \]
        }
        \subcase{$(x_{2k-1},y_{2k-1},\delta_{2k-1}) = (x'_{2k-1},y'_{2k-1},\delta'_{2k-1})$ and ($y'_{2k-1}=y$ and $x'_{2k-1}=\hat{x}$).}
        { If Bob updates, he performs a good update, and since $y'_{2k-1} = y$ and $x_{2k-1}=\hat{x}$, we have $\rho^B_{2k-1}=1$. He updates with probability $p_{2k-1}\geq 1-3\alpha_{2k-1}$, since the distance to the original message is at most the corruption. His probability is calculated as such because we are in the case where $y'_{2k-1} = y$ and $x_{2k-1}=\hat{x}$. Therefore, $\bbE [U_{2k-1}]\geq 1-3\alpha_{2k-1}$, and so $\bbE [U_{2k-1} - \min \{ \rho^B_{2k-1}, 0.5 \}]\geq 1-3\alpha_{2k-1}-0.5=0.5-3\alpha_{2k-1}$. (Note that we could've also had $U_{2k-1}=\rho^B_{2k-1}=0$ but then this expression trivially holds anyway.)
        
        Now, we evaluate $\bbE [\rho^A_{2k}+\Psi^A_k - \Psi_k]$. If $\psi^B_{2k-1} \ge N$, $\rho^A_{2k} = 1$, Bob must have updated positively, and he can only do so if he sends Alice a response of $\ECC(\hat{x},y_{2k-1},\delta)$ because of how the algorithm is defined. From the previous calculation we know $\bbE [\Psi^A_k - \Psi_k] \geq -3\alpha_{2k}$. If $\psi^B_{2k-1} \le N$, then $\rho^B_{2k}=0.5$, but $\bbE [\Psi^A_k - \Psi_k] \geq 0.5-3\alpha_{2k}$. Either way, $\bbE [\Psi^A_k - \Psi_k + U_{2k-1} + \rho^A_{2k}]\geq 1-3\alpha_{2k}$
        \[
            \bbE[\Psi^A_k - \Psi^A_{k-1}] = \bbE [\Psi^A_k - \Psi_k + U_{2k-1} - \min \{ \rho^B_{2k-1}, 0.5 \}+ \rho^A_{2k}] \geq 1-3\alpha_{2k}-3\alpha_{2k-1}=1-3\alpha_{2k-1}-3\alpha_{2k}.
        \]
        } \mnote{for the 2 subcases, we can't actually assert that if bob updates, he performs a bad update...}
        \subcase{$(x_{2k-1},y_{2k-1},\delta_{2k-1}) \neq (x'_{2k-1},y'_{2k-1},\delta'_{2k-1})$ and ($y_{2k-1}=y$ and $x_{2k-1}=\hat{x}$).}
        { If Bob updates, he performs a bad update. He updates with probability $p_{2k-1}\geq 1-3d$, where $d$ is the distance to $\ECC(x'_{2k-1},y'_{2k-1},\delta'_{2k-1})$. His probability is calculated as such because we are in the case where $y'_{2k-1}=y$ and $x'_{2k-1}=\hat{x}$. Note that $d\geq \frac12 -\alpha_{2k-1}$ since $\frac12$ is the smallest possible $\ECC$ distance. Then, $\bbE [U_{2k-1} - \min \{ \rho^B_{2k-1}, 0.5 \}]\geq 3d-1 - 0.5 \geq 1.5-3\alpha_{2k-1}-1.5=-3\alpha_{2k-1}$.
        
        Bob could only have performed a bad update, so $\psi^B_{2k-1} \le N$, and so $\rho^A_{2k}=0.5$ since $y_{2k-1}=y$, so $\bbE [\Psi^A_k - \Psi_k] \geq 0.5-3\alpha_{2k}$. Then, $\bbE [\Psi^A_k - \Psi_k + U_{2k-1} + \rho^A_{2k}]\geq 1-3\alpha_{2k}$ so
        \[
            \bbE[\Psi^A_k - \Psi^A_{k-1}] = \bbE [\Psi^A_k - \Psi_k + U_{2k-1} - \min \{ \rho^B_{2k-1}, 0.5 \}+ \rho^A_{2k}] \geq 1-3\alpha_{2k}-3\alpha_{2k-1}=1-3\alpha_{2k-1}-3\alpha_{2k}.
        \]
        }
        \subcase{$(x_{2k-1},y_{2k-1},\delta_{2k-1}) \neq (x'_{2k-1},y'_{2k-1},\delta'_{2k-1})$ and ($y_{2k-1}\neq y$ or $x_{2k-1}\neq \hat{x}$).}
        { If Bob updates, he performs a bad update. He updates with probability $p_{2k-1}\geq 0.5-3d$ (or 0), where $d$ is the distance to $\ECC(x'_{2k-1},y'_{2k-1},\delta'_{2k-1})$. His probability is calculated as such because we are in the case where $y_{2k-1}\neq y$ or $x_{2k-1}\neq \hat{x}$. Note that $d\geq \frac12 -\alpha_{2k-1}$ since $\frac12$ is the smallest possible $\ECC$ distance. Then, $\bbE [U_{2k-1} - \min \{ \rho^B_{2k-1}, 0.5 \}]\geq 3d-0.5 - 0.5 \geq 1.5-3\alpha_{2k-1}-1=0.5-3\alpha_{2k-1}$.
        
        Bob could only have performed a bad update, so $\psi^B_{2k-1} \le N$, so $\bbE [\Psi^A_k - \Psi_k] \geq 0.5-3\alpha_{2k}$. Note that $\rho^A_{2k}>0$, and $\bbE [\Psi^A_k - \Psi_k + U_{2k-1} + \rho^A_{2k}]\geq 0.5-3\alpha_{2k}$ so
        \[
            \bbE[\Psi^A_k - \Psi^A_{k-1}] = \bbE [\Psi^A_k - \Psi_k + U_{2k-1} - \min \{ \rho^B_{2k-1}, 0.5 \}+ \rho^A_{2k}] \geq 0.5-3\alpha_{2k}+0.5-3\alpha_{2k-1}=1-3\alpha_{2k-1}-3\alpha_{2k}.
        \]
        }
        \end{subcaseof}
    }
    \case{$\psi^B_{2k-2} \geq N$:} {
        We have 
        \begin{align*}
            \bbE[\Psi_k - \Psi^A_{k-1}] &= \bbE [\min \{ \psi^B_{2k-1}, N \} - \min \{ \psi^B_{2k-2} + \min \{ \rho^B_{2k-1}, 0.5 \}, N \} + \rho_{2k}^A] \\
            &= \bbE [\min \{ \psi^B_{2k-1}, N \} - N + \rho_{2k}^A]
        \end{align*}
    
        By Lemma~\ref{lemma:N}, Bob does know $x$ after message $2k-2$, so $x_{2k-2} = x$. 
        
        \begin{subcaseof}
        \subcase{$(x_{2k-1},y_{2k-1},\delta_{2k-1}) = (x'_{2k-1},y'_{2k-1},\delta'_{2k-1})$.}
        { If Bob updates, he performs a good update, and also $\hat{x}=x$. Therefore, $\psi^B_{2k-1}>N$ as well, so we are just computing $\bbE [\rho_{2k}^A]$. Bob sends $\ECC(\hat{x}=x,y_{2k-1}, \delta)$ with probability either $1-6\alpha_{2k-1}$ or $1-6\alpha_{2k}$, both of which are at least $1-6\alpha_{2k-1}$, which would give Alice an expected update of $1$. Otherwise, he sends $\ECC(\hat{x}=x,y,0)$ which might give Alice an expected update of 0.5. Thus, $\rho^A_{2k}\geq 1(1-6\alpha_{2k-1})+0.5(6\alpha_{2k-1})\geq 1-3\alpha_{2k-1}$. Then, $\bbE[\Psi_k - \Psi^A_{k-1}] \geq 1-3\alpha_{2k-1}$. Then,
        
        \[
            \bbE[\Psi^A_k - \Psi^A_{k-1}] = \bbE [\Psi^A_k - \Psi_k + \Psi_k - \Psi^A_{k-1}] \geq -3\alpha_{2k}+1-3\alpha_{2k-1}=1-3\alpha_{2k-1}-3\alpha_{2k}.
        \]
        }
        \subcase{$(x_{2k-1},y_{2k-1},\delta_{2k-1}) \neq (x'_{2k-1},y'_{2k-1},\delta'_{2k-1})$ and ($y_{2k-1}=y$ and $x_{2k-1}=\hat{x}$).}
        { If Bob updates, he performs a bad update. He updates with probability $p_{2k-1}\geq 1-3d$, where $d$ is the distance to $\ECC(x'_{2k-1},y'_{2k-1},\delta'_{2k-1})$. His probability is calculated as such because we are in the case where $y'_{2k-1}=y$ and $x'_{2k-1}=\hat{x}$. This corresponds exactly to when he sends $\ECC(\hat{x},y_{2k-1}=y,\delta)$ to Alice. If he doesn't update, he sends $\ECC(\hat{x},y,0)$ to Alice. Both these cause Alice to update at least $0.5$ in expectation if uncorrupted.
        
        In the first case, $\bbE [\min \{ \psi^B_{2k-1}, N \} - N + \rho_{2k}^A]$ can be as low as $N-1-N+0.5=-0.5$. In the second case, it is $N-N+0.5=0.5$. Thus, in expectation, it is $-0.5(1-3d)+0.5(3d)=3d-0.5$. Note that $d\geq \frac12 -\alpha_{2k-1}$ since $\frac12$ is the smallest possible $\ECC$ distance. Then, $\bbE [\min \{ \psi^B_{2k-1}, N \} - N + \rho_{2k}^A] \geq 3d-0.5 \geq 1.5-3\alpha_{2k-1}-0.5=1-3\alpha_{2k-1}$. Then,
        \[
            \bbE[\Psi^A_k - \Psi^A_{k-1}] = \bbE [\Psi^A_k - \Psi_k + \Psi_k - \Psi^A_{k-1}] \geq -3\alpha_{2k}+1-3\alpha_{2k-1}=1-3\alpha_{2k-1}-3\alpha_{2k}.
        \]
        }
        
        \subcase{$(x_{2k-1},y_{2k-1},\delta_{2k-1}) \neq (x'_{2k-1},y'_{2k-1},\delta'_{2k-1})$ and ($y_{2k-1}\neq y$ or $x_{2k-1}\neq \hat{x}$).}
        { If Bob updates, he performs a bad update. He updates with probability $p_{2k-1}\geq 0.5-3d$, where $d$ is the distance to $\ECC(x'_{2k-1},y'_{2k-1},\delta'_{2k-1})$. His probability is calculated as such because we are in the case where $y_{2k-1}\neq y$ or $x_{2k-1}\neq \hat{x}$. He will send $\ECC(\hat{x},y_{2k-1},\delta)$ to Alice with $q_{2k-1}=1-6d$, or $\ECC(\hat{x},y,0)$ to Alice with probability $6d$.
        
        Then, in expectation $\rho_{2k}^A$ is at least $0(1-6d)+0.5(6d)=3d$. Also, $\bbE [\min \{ \psi^B_{2k-1}, N \} - N]$ is at least $-1(0.5-3d)+0(0.5+3d)=-0.5+3d$. These two terms add to $6d-0.5$. Note that $d\geq \frac12 -\alpha_{2k-1}$ since $\frac12$ is the smallest possible $\ECC$ distance. Then, $\bbE [\min \{ \psi^B_{2k-1}, N \} - N + \rho_{2k}^A] \geq 6d-0.5 \geq 3d-0.5 \geq 1.5-3\alpha_{2k-1}-0.5=1-3\alpha_{2k-1}$. Then,
        \[
            \bbE[\Psi^A_k - \Psi^A_{k-1}] = \bbE [\Psi^A_k - \Psi_k + \Psi_k - \Psi^A_{k-1}] \geq -3\alpha_{2k}+1-3\alpha_{2k-1}=1-3\alpha_{2k-1}-3\alpha_{2k}.
        \]
        }
        
        \end{subcaseof}
    }
    \end{caseof}
    
\end{proof}
    
\begin{proof}[Proof of Theorem~\ref{thm:1/6}]
    Let $\alpha_0, \dots, \alpha_{T}$ denote the fractional number of corruptions in messages $0, \dots, T$, such that $\alpha_0 + \dots + \alpha_{T} < \left( \frac16 - \epsilon \right) \cdot T$. By default, we let $\alpha_0 = 0$. For $k \in [T/2]$, we define the random variables
    \begin{align*}
        \Phi^A_k &= \Psi^A_k - k + \sum_{i=0}^{2k} 3\alpha_i, \\
        \Phi^B_k &= \Psi^A_k - k + \sum_{i=0}^{2k-1} 3\alpha_i.
    \end{align*}
    Then, $\Phi^A_0 = \Psi^A_0 \in \{ 0.5, 1.5 \}$ and $\Phi^B_0 = \Psi^B_0 = 0.5$.
    
    By Lemma~\ref{lemma:0.5-3alpha}, 
    \begin{align*}
        \bbE[\Psi^A_k] &\ge \bbE[\Psi^A_{k-1}] + 1 - 3\alpha_{2k-1} - 3\alpha_{2k} \\
        \implies \bbE[\Phi^A_k] &= \bbE \left[ \Psi^A_k - k + \sum_{i=0}^{2k} 3\alpha_i \right] \\
        &\ge \bbE \left[ \Psi^A_{k-1} - (k-1) + \sum_{i=0}^{2k-2} 3\alpha_i \right] \\
        &= \bbE[\Phi^A_{k-1}],
    \end{align*}
    so $\Phi^A_k$ is a submartingale with bounded distance 
    \[
        |\Phi^A_k - \Phi^A_{k-1}| 
        = \left| \Psi^A_k - \Psi^A_{k-1} - 1 + 3\alpha_{2k-1} + 3\alpha_{2k} \right|
        < 10.
    \]
    Similarly, $\Phi^B_k$ is a submartingale with bounded distance $< 10$.
    
    Note that if $\Psi^A_{T/2} \ge 2N$, then $\psi^A_T = \Psi^A_{T/2} - \min \{ \psi^B_T, N \} \ge N$, meaning by Lemma~\ref{lemma:N} that Alice holds $\hat{y} = y$ at the end of the protocol. Thus, the probability that Alice outputs correctly at the end of the protocol is at least
    \begin{align*}
        \Pr \left[ \Psi^A_{T/2} \ge 2N \right]
        &= 1 - \Pr \left[ \Phi^A_{T/2} - \Phi^A_0 < 2N - \Phi^A_0 - \frac{T}{2} + \sum_{i=0}^{T} 3\alpha_i \right] \\
        &\ge 1 - \Pr \left[ \Phi^A_{T/2} - \Phi^A_0 < 2N - \frac{T}{2} + 3 \cdot \left( \frac16 - \epsilon \right) \cdot T \le -N \right] \\
        &\ge 1 - \exp \left( \frac{-\epsilon N}{100} \right).
    \end{align*}
    The same calculation for Bob shows that Bob outputs correctly at the end of the protocol with probability at least $1 - \exp \left( \frac{-\epsilon N}{100} \right)$ as well. Then by a union bound, the probability that both parties output correctly is at least
    \[
        1 - 2 \cdot \exp \left( \frac{-\epsilon N}{100} \right).
    \]
    
\end{proof}

==> toggle/1.6-orig/protocol.tex <==
\subsection{Protocol}

\protocol{Randomized Protocol Resilient to $\frac16 - \epsilon$ Corruptions}{1/6}{
    Suppose Alice and Bob's private inputs are $x,y \in \{ 0, 1 \}^{n} = [1, N]$, where $N = 2^n$. Let $\ECC : [0, N] \times [0, N] \times \{ -1, 0, +1 \} \rightarrow \{ 0, 1 \}^M$ be an error correcting code such that for any $(x_0, y_0, \delta_0)$ and $(x_1, y_1, \delta_1)$ such that $x_0 \not= x_1 ~\vee~ y_1 \not= y_0$, $\Delta(\ECC(x_0, y_0, \delta_0), \ECC(x_1, y_1, \delta_1)) \ge \frac{M}{2}$, and for any $\delta_0 \not= \delta_1$, $\Delta(\ECC(x_0, y_0, \delta_0), \ECC(x_0, y_0, \delta_1)) = \frac23 M$.
    
    The protocol consists of $T = \frac{N}{\epsilon}$ (assume $T$ is even) messages numbered $1, \dots, T$, each of length $M$. Alice sends the odd messages and Bob sends the even. Alice and Bob each keep track of a private guess for the other party's input, denoted $\hat{y} \in [0,N_B]$ and $\hat{x} \in [0,N_A]$ respectively. $\hat{x}$ and $\hat{y}$ are both initialized at $0$. They also each have a personal counter $c_A$ and $c_B$ respectively, initialized at $0$. The behavior of Alice and Bob is symmetric. In what follows, we describe Alice's behavior.
    
    \begin{itemize}
        
    \item 
        Alice has just received a message $m$ from Bob. For convenience, we consider the $0$'th message to be $\ECC(0,0,+1)$, sent uncorrupted by Bob to Alice.
        \mnote{We need to design an ECC so computing this decoding is easy.}
        For each possible triple $(x', y', \delta')$ with $x'\in [N], y' \in [N], \delta' \in \{ -1, 0, +1 \}$, let 
        \[
            d(x', y', \delta') = \frac{\Delta(m, \ECC(x', y', \delta'))}{M}
        \]
        i.e. $d(x',y',\delta')$ is the relative distance from $m$ to $\ECC(x', y', \delta')$. Define $b(x', y')=1$ if $x'=x ~\wedge~ y' = \hat{y}$ and $b(x', y')=0$ otherwise. We define
        \[
            p(x', y', \delta') = \frac{1 + b(x', y')}2 - 3d(x', y', \delta')
        \]
        and
        \[  
            q(x', y', \delta') = 1-(6-3b(x', y'))\cdot d(x', y', \delta').
        \]
        
        By Lemma~\ref{onep}, $p$ and $q$ are each positive for at most one triple $(x', y', \delta')$, and if such a triple exists, it must be the same triple for both $p$ and $q$ with $q \ge p$. If it exists, let this triple be $(x_B, y_B, \delta_B)$, and define $p_B = \{ p(x_B, y_B, \delta_B)$ and $p_Q = \{ q(x_B, y_B, \delta_B)$, such that $q_B \ge p_B > 0$. If no such triple $(x_B, y_B, \delta_B)$ exists, then we let $p_B = q_B = 0$.
        
        Alice picks a real number $r \in [0, 1]$ uniformly at random.
        
        \begin{center}
            {\bf Update Phase}
        \end{center}
        
        \begin{itemize}
        \item 
            If $r \le p_B$ and $y_B = \hat{y}$, she performs the following update:
            \begin{itemize}
                \item If $\delta_B = 0$, she updates $c_A \gets c_A + 1$ and does nothing to $\hat{y}$.
                \item If $\delta_B \in \{ -1, +1 \}$ and $c_A > 0$, she updates $c_A \gets c_A - 1$ and does nothing to $\hat{y}$.
                \item If $\delta_B \in \{ -1, +1 \}$ and $c_A = 0$, she updates $\hat{y} \gets \hat{y} + \delta_B$.
            \end{itemize}
        \item 
            If $r \le p_B$ and if$y_B \not= \hat{y}$ and $\delta_B = 0$, she does the following update:
            \begin{itemize}
                \item If $c_A > 0$, she updates $c_A \gets c_A - 1$ and does nothing to $\hat{y}$.
                \item If $c_A = 0$, let $\delta = \sign(y_B - \hat{y})$. She updates $\hat{y} \gets \hat{y} + \delta$.
            \end{itemize}
        \item 
            Any other case where $r > p_B$ or $y_B \not= \hat{y}$ she does nothing.
        \end{itemize}
        
        \begin{center}
            {\bf Send Phase}
        \end{center}
        
        \begin{itemize}
            \item If $r \le q_B$, Alice does the following: If $x_{B} = x$, let $\delta_A = 0$. Otherwise, let $\delta_A = \sign(x-x_{B})$. Alice sends $\ECC(x_{B}, \hat{y}, \delta_A)$. 
            \item Otherwise, $r > q_B$, and she sends $\ECC(x,\hat{y},0)$.
        \end{itemize}
        
    \item 
        At the end of the protocol, Alice outputs $\hat{y}$.
        
    \end{itemize}
}

==> toggle/1.7-inefficient.tex <==
\subsection{$1/7$ Construction (Inefficient)}


\protocol{Two Way Inefficient Protocol Resilient to $1/7-\epsilon$ Corruptions}{coin}{
    Let the two inputs be length $n$. Let $N=\frac{n}{\epsilon}$. Define $ECC(y, S_1, S_2, S_3)$, where $y\in \{0,1\}^n$, and $S_1, S_2, S_3$ is a partition of the set of all possible $x$. This ECC is length $4M$.
    
    The protocol consists of $N$ chunks, where Bob sends $4M$ messages and Alice sends $3M$ messages.
    
    In each chunk, Bob asks a question, and Alice responds.
    
    \begin{itemize}
        \item \textbf{Bob:} Bob tracks an internal state assigning all possible values of $x$ to a number, representing his estimate of lies told so far if that is the true value of $x$. Denote this $l(x_i)$. Order the $x_i$ by $l$, and denote them in order $l_1\ldots l_N$. Let $S_1=\{l_1\}$, $S_2=\{x_2,x_4\ldots\}$ and $S_3=\{x_3,x_5\ldots\}$. Send $ECC(y,S_1,S_2,S_3)$.
        
        \item \textbf{Alice:} Alice decodes Bob's message to $y, S_1, S_2, S_3$ (which may not be accurate). Bob's message is distance $k$ from the encoding of her decoding (estimate of lies). If $x$ is in $S_1$, she sends $M$ 1's followed by $2M$ 0's. If it's in $S_2$, she sends $M$ 0's, followed by $M$ 1's, followed by $M$ 0's. If it's in $S_3$, she sends $2M$ 0's followed by $M$ 1's. However, she replaces $k$ of the 1's with 0's arbitrarily.
        
        \item \textbf{Bob:} Bob increases the lie estimate $l(x_i)$ for everything in $S_1$ according to the distance to $1^M0^{2M}$, and same for $S_2$ and $S_3$. Note that this is based on $S_i$ as he sent them, not how Alice decoded them.
    \end{itemize}
    
    At the end, Alice decodes $y$ by looking at the $y$ that caused the least lies over all possible messages Bob sent.
    
    Bob guesses $l_1$.
}

\begin{lemma}\cite{SpencerW92}
    For all $\delta > 0$ there is a constant $c > 0$ such that if $t > c \log n$ then the leftmost chip is at least at position $\frac{1-\delta}2 \cdot t$.
\end{lemma}


==> toggle/1.7-randomized.tex <==
\subsection{$1/7$ Construction (Randomized)}


\protocol{Two Way Randomized Protocol Resilient to $1/7-\epsilon$ Corruptions}{rewind-if-error}{
    Consider the message exchange task where Alice has input $x$ of size $n_A$ and Bob has input $y$ of size $n_B$. Let $N = \frac{3n_A}{\epsilon}$ and let $\tilde{x}$ denote $x || 0^{N - n_A}$. Let $\ECC(\cdot, \cdot) : \{ 0, 1 \}^{n_B} \times \{ 0, 1, \emptyset \}^N \rightarrow \{ 0, 1 \}^K$ be an error correcting code with distance $\frac12 - \epsilon$. Let $M = (\frac14 - \frac\epsilon2) \cdot K$.
    
    Our error-resilient protocol consists of $N$ chunks where Bob speaks $K$ rounds, followed by Alice speaking $3M$ rounds. 
    \begin{itemize}
    \item 
        In each chunk, Bob sends $\ECC(y, X)$ ($X$ is a string of $0$'s and $1$'s and is padded with $\emptyset$'s if it is shorter than $N)$, where $X$ is constructed as follows: Initially, $X = \emptyset$. When Bob receives $m \in \{ 0, 1 \}^{3M}$ from Alice, he picks an index $i \in [3M]$ uniformly at random. If $m[i] = 0$, he does nothing. Otherwise, if $i \le M$ and $m[i] = 1$, he appends a $0$ to $X$. If $M < i \le 2M$ and $m[i] = 1$, he appends a $1$ to $X$. Finally, if $2M < i$ and $m[i] = 1$, he removes the last character from $X$ (if $X$ is already empty, he does nothing). In other words, when Bob receives $m \in \{ 0, 1 \}^{3M}$ from Alice consisting of $a$ $1$'s in the first $M$ bits, $b$ $1$'s in the second $M$ bits, and $c$ $1$'s in the third $M$ bits, he:
        \begin{itemize}
            \item adds a $0$ to the end of $X$ with probability $\frac{a}{3M}$, 
            \item adds a $1$ to the end of $X$ with probability $\frac{b}{3M}$, and
            \item removes the last symbol from the end of $X$ with probability $\frac{c}{3M}$,
        \end{itemize}
        and otherwise does not alter $X$ at all.
    \item 
        When it's Alice's turn to speak and she has just received Bob's message $\ct \in \{ 0, 1 \}^K$, she decodes to get $(y', X') \in \{ 0, 1 \}^{n_B} \times \{ 0, 1, \emptyset \}^N$ and calculates $t = \Delta(\ct, \ECC(y', X')$. If $t \ge M$ or $X'$ is malformed (i.e. it is not a collection of $1$'s and $0$'s followed by $\emptyset$'s), she sends $0^{3M}$. Otherwise, letting $X''$ denote the prefix of $X'$ consisting only of $0$'s and $1$'s, if $X''$ is also a prefix of $\tilde{x}$, Alice sends $1^M 0^{2M}$ if the next bit of $\tilde{x}$ is a $0$ and $0^M 1^M 0^M$ if the next bit of $\tilde{x}$ is a $1$. If $X''$ is not a prefix of $\tilde{x}$, Alice sends $0^{2M} 1^M$. 
    \end{itemize}
    
    At the end of the protocol, Alice outputs $(x, \hat{y})$ where $\hat{y} \in \{ 0, 1 \}^{n_B}$ is such that there exists $X_1, \dots, X_N$ satisfying $\sum_{i \in [N]} \Delta(\ct_i, \ECC(\hat{y}, X_i)) < \frac{n_A}{\epsilon} \cdot M$ (if such $\hat{y}$ doesn't exist, Alice outputs arbitrarily). Bob outputs $(\hat{x}, y)$, where $\hat{x}$ is the first $n_A$ bits of $X$.
}
    
    
\begin{theorem}
    The protocol given in Figure~\ref{fig:1/7-randomized} is resilient to a $\frac17 - \epsilon$ fraction of adversarial bit flips with probability $1 - e^{-\Omega(n_A)}$.
\end{theorem}

\begin{proof}
    First, note that a $\frac17 - \epsilon$ fraction of corruptions is 
    \begin{align*}
        \left( \frac17 - \epsilon \right) \cdot N (K + 3M) 
        &\le \left( \frac17 - \epsilon \right) \cdot \left( \frac{4}{1-2\epsilon} + 3 \right) \cdot NM \\
        &= \left( \frac17 - \epsilon \right) \cdot \left( 7 + \frac{8\epsilon}{1-2\epsilon} \right) \cdot NM \\
        &\le (1-2\epsilon) NM
    \end{align*}
    corruptions. We will show that the protocol is resilient to any adversarial corruption of $(1-2\epsilon) NM$ bits, which is a stronger statement than the theorem statement. For the rest of this proof, we assume that an adversary makes at most $(1-2\epsilon) NM$ corruptions.
    
    Note that if at most $(1-2\epsilon) NM$ corruptions are made, then in particular at most $NM = (\frac14 - \frac\epsilon2) \cdot NK$ corruptions are made to Bob's messages, so $\hat{y} = y$ satisfies Alice's output condition. Furthermore, $y$ is the only such value of $\hat{y}$ satisfying Alice's output condition; otherwise, if there exist $y'$ and $X_1, \dots, X_N, X'_1, \dots, X'_N$ such that 
    \[
        \sum_{i \in [N]} \Delta(\ct_i, \ECC(y, X_i)) < N M
    \]
    and
    \[
        \sum_{i \in [N]} \Delta(\ct_i, \ECC(y', X'_i)) < N M,
    \]
    then adding these and applying triangle inequality gives
    \begin{align*}
        \sum_{i \in [N]} \Delta(\ECC(y, X_i), \ECC(y', X'_i)) 
        &\le \sum_{i \in [N]} \Delta(\ct_i, \ECC(y, X_i)) + \sum_{i \in [N]} \Delta(\ct_i, \ECC(y', X'_i)) \\
        &< \left( \frac12 - \epsilon \right) \cdot N K,
    \end{align*}
    so in particular there exists $i \in [N]$ for which $\Delta(\ECC(y, X_i), \ECC(y', X'_i)) < (\frac12 - \epsilon) \cdot K$, which is not possible as the minimum relative distance of $\ECC$ is $\frac12 - \epsilon$. So Alice will always learn Bob's input correctly.
    
    We now show that Bob learns Alice's input with high probability as well. At the beginning of a chunk, right after Bob has heard $3M$ bits from Alice, we say that his next operation to $X$ is \emph{good} if either $X$ is currently a prefix of $\tilde{x}$ and the operation is appending the next bit of $\tilde{x}$ to $X$, or if $X$ is not a prefix of $\tilde{x}$ and the operation is removing the last bit of $X$. Otherwise, if he does nothing to $X$, his operation is \emph{neutral}; in any other case it is \emph{bad}. Note that at the end of the protocol, as long the number of good operations is $n_A$ more than the number of bad operations performed, the prefix of $X$ of size $n_A$ is equal to $x$ and Bob outputs correctly. (To see this, note that any bad operation requires one good operation to reverse.)
    
    Let $\Phi(i)$ denote the number of good operations minus the number of bad operations done so far at the end of the $i$'th chunk (including the most recent one done in response to Alice's most recent messages). 
    
    \begin{claim} \label{claim:Phi(i)}
        If the adversary corrupts $e$ messages in chunk $i$, then $\mathbb{E} \left[ \Phi(i) - \Phi(i-1) \right] \ge \frac13 - \frac{e}{3M}$.
    \end{claim}
    
    \begin{proof}
        Note that if the adversary corrupts none of the messages in a chunk, then Alice sends two sets of $M$ $0$'s corresponding to the bad operations and $M$ $1$'s corresponding to the good operation. This means that with probability $\frac13$ Bob performs a good operation and with probability $\frac23$ does nothing at all. We show that each additional corruption by the adversary to either Bob's or Alice's messages either decreases the probability that Bob performs a good operation by $\le \frac{1}{3M}$ or increases the probability that Bob performs a bad operation by $\le \frac{1}{3M}$. 
        
        First, each of the first $(\frac14 - \frac\epsilon2) K$ corruptions to Bob's messages results in one fewer $1$ that Alice sends corresponding to the good operation, i.e. each corruption to one of Bob's messages results in a $\frac1{3M}$ decrease in the probability that Bob performs a good operation. Any additional corruption to Bob's messages either does not change Alice's response (in the case that the distance of $\ct_i$ to any possible codeword is too high, or decoding results in a malformed $X'$) or increases the number of $1$'s corresponding to a bad operation by $1$ (in the case that $\ct_i$ is now closer to an incorrect codeword encoding a well-formed $y'$ and $X'$). 
        
        Regardless of the number or pattern of corruptions done onto Bob's messages, any corruption to Alice's messages affects the probability that Bob performs a good or bad operation by $\frac{1}{3M}$ either positively or negatively. In particular, it decreases the probability that Bob performs a good operation by at most $\frac1{3M}$ and increases the probability that Bob performs a bad operation by at most $\frac{1}{3M}$.
        
        In total, each corruption affects the expected value of $\Phi(i) - \Phi(i-1)$ by at most $-\frac{1}{3M}$. 
    \end{proof}
    
    Let $e_1, \dots, e_N$ denote the number of corruptions in chunks $1, \dots, N$. 
    Define the random variable $\Psi(i) := \Phi(i) + \frac{\sum_{j=1}^i e_j}{3M} - \frac{i}{3}$ (where $\Psi(0) := 0$). By Claim~\ref{claim:Phi(i)}, 
    \begin{align*}
        \bbE \left[ \Phi(i) \right] + \frac{e_i}{3M} - \frac13 
        &\ge \bbE \left[ \Phi(i-1) \right] \\
        \implies \bbE [ \Psi(i) ] 
        &= \bbE \left[ \Phi(i) + \frac{\sum_{j=1}^i e_j}{3M} - \frac{i}{3} \right] \\
        &\ge \bbE \left[ \Phi(i-1) + \frac{\sum_{j=1}^{i-1} e_j}{3M} - \frac{i-1}{3} \right] \\
        &= \bbE [ \Psi (i-1) ],
    \end{align*}
    so $\Psi(i)$ is a submartingale with bounded \rnote{I am rusty on martingales and exactly what they are... Yael, could you read over this proof and make sure it's correct when you get a chance?} difference 
    \[
        |\Psi(i) - \Psi(i-1)| 
        = \left| \Phi(i) - \Phi(i-1) + \frac{e_i}{3M} - \frac13 \right| 
        < 1 + \frac{K + 3M}{3M}  - \frac13
        < 1 + \frac83 - \frac13
        = \frac{10}{3}. 
    \]
    Then, by Azuma's inequality, Bob learns Alice's input correctly with probability
    \begin{align*}
        \Pr \left[ \Phi(N) \ge n_A \right]
        &= 1 - \Pr \left[ \Psi(N) - \Psi(0) < n_A + \frac{\sum_{j=1}^N e_j}{3M} - \frac{N}{3} \right] \\
        &\ge 1 - \Pr \left[ \Psi(N) - \Psi(0) < n_A + \frac{(1-2\epsilon) NM}{3M} - \frac{N}{3} = -n_A \right] \\
        &\ge 1 - \exp \left( \frac{-n_A^2}{2N \cdot (\frac{10}{3})^2} \right) \\
        &= 1 - \exp \left( \frac{-9\epsilon n_A}{50} \right).
    \end{align*}
\end{proof}



% \begin{figure}[h!]
%     \centering
%     \protocol{}{
%         Let $\pi_0$ be a noiseless, interactive, two-party protocol with a fixed order of speaking. We may assume that $\pi_0$ has an alternating speaking order with at most a $2\times$ blowup in the communication complexity. Suppose that each party speaks $n_0$ rounds, for a total of $2n_0$ rounds, with Bob speaking first speaking first. Extend the protocol to $\frac{2n_0}{\epsilon}$ rounds by having both parties send $0$ in each round they speak past the first $2n_0$ (the protocol should still be alternating). 
        
%         Let $\ECC(\cdot, \cdot) : \{ 0, 1, \emptyset \}^{2n_0/\epsilon} \rightarrow \{ 0, 1 \}^{4M}$ be an error correcting code with distance $\frac12 - \epsilon$. 
        
%         Our error-resilient protocol consists of $\frac{2n_0}{\epsilon}$ chunks where Bob speaks $4M$ rounds, followed by Alice speaking $3M$ rounds. 
%         \begin{itemize}
%             \item 
%         \end{itemize}
%     }
%     \caption{Two Way Randomized Protocol Resilient to $1/7-\epsilon$ Corruptions}
%     \label{fig:1/7-randomized}
% \end{figure}



==> toggle/old.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% MESSAGE-BASED POTENTIAL %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In each chunk, Alice and Bob each send a message of $M$ bits. Number these messages from $1$ to $2T$, such that Alice's message in the $t$'th chunk is message $2t + 1$ and Bob's message in the $t$'th chunk is message $2t+2$. For each message $k \in [0, 2T]$, we define the following potential functions:
\begin{itemize}
    \item $\psi^A_k$ is the number of good updates minus the number of bad updates Alice has done in response to messages $1, \dots, k$, plus the expected number of good updates minus bad updates she will have done in response to message $k+1$ (only nonzero if Bob sends message $k+1$), assuming no corruptions are made to message $k+1$. If $k = 2T$, then $\psi_A^{2T}$ is just the number of good updates minus the number of bad updates Alice has done the entire protocol.
    \item $\psi^B_k$ is analogously defined as the number of good updates minus the number of bad updates Bob has done in response to messages $1, \dots, k$, plus the expected number of good minus bad updates he will have done in response to message $k+1$, assuming message $k+1$ is uncorrupted. If $k = 2T$, then $\psi_B^{2T}$ is just the number of good updates minus the number of bad updates Bob has done the entire protocol.
\end{itemize}
For instance, if $k = 0$, $\psi^A_0 = \psi^B_0 = 0.5$.

\noindent
We also define the following two potential functions, for each $k \in [0, 2T]$:
\begin{itemize}
    \item $\Psi^A_k = \psi^A_k + \min \{ N+1, \psi^B_k \}$.
    \item $\Psi^B_k = \psi^B_k + \min \{ N+1, \psi^A_k \}$.
\end{itemize}
Then, $\Psi^A_0 = \Psi^B_0 = 1$.

\begin{claim} \label{claim:0.5-3alpha}
    If $\alpha$ fraction of message $k$ is corrupted, then 
    \[
        \bbE [\Psi^A_k - \Psi^A_{k-1}] \ge \max \{ 0.5 - 3\alpha, -1 \}
    \]
    and
    \[
        \bbE [\Psi^B_k - \Psi^B_{k-1}] \ge \max \{ 0.5 - 3\alpha, -1 \}.
    \]
\end{claim}

\begin{proof}
    Without loss of generality, we assume Alice sent message $k$ to Bob. Let the message be $m$. 
    Notice that $\bbE [\psi^A_k - \psi^A_{k-1}]$ is just Alice's expected good minus bad update in response to message $k+1$ if it is uncorrupted, since she makes no updates or is expected to after message $k$. This value is at least $0.5-\alpha$.
    
    Notice that $\bbE [\psi^B_k - \psi^B_{k-1}]$ is Bob's expected update after message $k$ with the $\alpha$ corruptions, minus his expected update with no corruptions. This value is at least $-3\alpha$.
    
    Also $\bbE [\psi^A_k - \psi^A_{k-1} + \psi^B_k - \psi^B_{k-1}] > 0.5-3\alpha$.
    
    \mnote{need to explain all the calculations}
    
    We will first show \[
        \bbE [\Psi^A_k - \Psi^A_{k-1}] \ge \max \{ 0.5 - 3\alpha, -1 \}
    \]. 
    \begin{caseof}
        \case {$\psi_k^B>N+1$ and $\psi_{k-1}^B>N+1$.}
            {We have $$\bbE [\Psi^A_k - \Psi^A_{k-1}] = \bbE [\psi^A_k - \psi^A_{k-1}]>0.5-\alpha$$ which is just Alice's expected good minus bad update in response to message $k+1$ uncorrupted. This is clearly $>-1$ since no one update can be worse than $-1$.}
        \case {$\psi_k^B<N+1$ and $\psi_{k-1}^B<N+1$.}
            {We have $$\bbE [\Psi^A_k - \Psi^A_{k-1}] = \bbE [\psi^A_k - \psi^A_{k-1} + \psi^B_k - \psi^B_{k-1}] > 0.5-3\alpha$$ by the above calculation
            }
    \end{caseof}
\end{proof}

For the rest of this proof, we will assume that the adversary makes fewer than $(\frac16 - \epsilon) \cdot 2M T$ corruptions. Assuming this, we will show that Alice ends the protocol with the value $\hat{y} = y$ with high probability. The analysis for Bob is equivalent.

Let $\alpha_1, \dots, \alpha_{2T}$ denote the fractional number of corruptions in the messages $1, \dots, 2T$, such that $\alpha_1 + \dots + \alpha_{2T} < (\frac16 - \epsilon) \cdot 2 T$. For $k = 1, \dots, 2T$, define the random variable $\Phi^A_{k} = \Psi^A_k - \frac{k}{2} + \sum_{i=1}^k 3\alpha_i$. By Claim~\ref{claim:0.5-3alpha}, 
\begin{align*}
    \bbE [\Psi^A_k] - 0.5 + 3\alpha_k &\ge \bbE [\Psi^A_{k-1}] \\
    \implies \bbE [\Phi^A_k] &= \bbE \left[ \Psi^A_k - \frac{k}{2} + \sum_{i=1}^k 3\alpha_i \right] \\
    &\ge \bbE \left[ \Psi^A_{k-1} - \frac{k-1}{2} + \sum_{i=1}^{k-1} 3\alpha_i \right] \\
    &= \bbE [\Phi^A_{k-1}]
\end{align*}
so $\Phi^A_k$ is a submartingale with bounded difference 
\[
    \left| \Phi^A_k - \Phi^A_{k-1} \right|
    = \left| \Psi^A_k - \Psi^A_{k-1} - \frac12 + 3\alpha_k \right| 
    \le 2 + 2.5 
    < 5.
\]
\rnote{prolly should say why the above is true}
Note that if $\Psi^A_{2T} \ge 2N+2$, then $\psi^A_k \ge N+1$, meaning that Alice holds $\hat{y} = y$ at the end of the protocol. Thus, the probability that Alice outputs correctly is at least 
\begin{align*}
    \Pr \left[ \Psi^A_{2T} \ge 2N+2 \right]
    &= 1 - \Pr \left[ \Phi^A_{2T} - \Phi^A_0 < 2N+1 - T + \sum_{i=1}^{2T} 3\alpha_i \right] \\
    &\ge 1 - \Pr \left[ \Phi^A_{2T} - \Phi^A_0 < 2N+1 - T + 3 \cdot \left( \frac16 - \epsilon \right) \cdot 2T \le -3N \right] \\
    &\ge 1 - \exp\left( \frac{- 9 \epsilon N}{100} \right).
\end{align*}

The above analysis holds for Bob as well. Thus, by a union bound on the probability of error, both Alice and Bob correctly output the other's output with probability at least $1 - 2 \exp\left( \frac{- 9 \epsilon N}{100} \right)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% ATTEMPT AT PROVING WRONG CHUNK POTENTIAL %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{proof}
        
    We only prove the first claim for Alice, as the proof for Bob is identical.
    
    We note that $\bbE [\psi_{2k}^A-\psi_{2k-2}^A]$ is Alice's expected update to message $2k$ given its corruption.
    
    We note that $\bbE [\psi_{2k}^B-\psi_{2k-2}^B]$ is Bob's expected update to message $2k+1$ with no corruption plus expected update to $2k-1$ with corruption minus expected update to $2k-1$ without corruption.
    
    Let $\rho_{t}$ if $t$ odd be Bob's expected update to message $t$ with corruption minus the expected update without corruption, plus Alice's expected update to message $t+1$ if it is uncorrupted. Finally, add $0.5$ if $\hat{y}=y$ after message $t+1$ uncorrupted. Define $\rho_t$ for even $t$ similarly.
    
    Let $\ECC(x_{2k-1},y_{2k-1},\delta_{2k-1})$ be the what Alice sent as message $2k-1$ and $\ECC(x_{2k},y_{2k},\delta_{2k})$ be the what Bob sent as message $2k$. Upon receiving the respective messages, Bob and Alice respecitvely will calculate $p_{2k-1}, q_{2k-1}, \ECC(x_{2k-1},y_{2k-1},\delta_{2k-1})$ and $p_{2k}, q_{2k}, \ECC(x_{2k},y_{2k},\delta_{2k})$ as in Lemma~\ref{onep}.
    
    \begin{claim}
        If $t$ is odd, and Bob is wrong about $x$ after updating from message $t$, then $\rho_t\geq 0.5-3\alpha_t$. Similarly, if $t$ is even and Alice is wrong about $x$ after updating from message $t$, then $\rho_t\geq 0.5-3\alpha_t$.
    \end{claim}
    
    \begin{proof}
        We only show the $t$ odd case; the even case follows analogously.
        
        Let $\ECC(x_t,y_t,\delta_t)$ be the what Alice sent as message $2k-1$ and $\ECC(x_{t+1},y_{t+1},\delta_{t+1})$ be the what Bob sent as message $t+1$. Upon receiving the respective messages, Bob and Alice respecitvely will calculate $p_{t}, q_{t}, \ECC(x'_{t},y'_{t},\delta'_{t})$ and $p_{t+1}, q_{t+1}, \ECC(x'_{t+1},y'_{t+1},\delta'_{t+1})$ as in Lemma~\ref{onep}.
        
        \begin{caseof}
        \case{$(x_{t},y_{t},\delta_{t})=(x'_{t},y'_{t},\delta'_{t})$.}
        {
            Then, Bob's chance of choosing the message changed from $0.5$ or $1$ to at least $0.5-3\alpha_{t}$ or $1-3\alpha_t$ respectively. In either case, this is a decrease of at most $3\alpha_t$. The message either gains Bob 1 progress or 0 progress if chosen (since Alice will never send a message signaling a bad update) so the total expected progress only decreases by $3\alpha_t$. The message Bob responds with will always be either $\ECC(\hat{x},y_t,?)$ or $\ECC(\hat{x},y,?)$. Since Bob is not right about $\hat{x}$, both of these would cause Alice to update 0.5 in expectation. Thus, $\rho_t\geq 0.5-3\alpha_t$.
        }
        \case{$(x_{t},y_{t},\delta_{t})\neq(x'_{t},y'_{t},\delta'_{t})$.}
        {
            The distance to $(x'_{t},y'_{t},\delta'_{t})$ will be $d$, so Bob's probability choosing it is $0.5b(y'_t)+0.5-3d$. 
            \begin{subcaseof}
            \subcase{$y_t=y, y'_t=y$.}
            {Then $d>\frac23-\alpha_t$. Bob's update with no corruption was expected to be $1$, Bob's actual update will be at least $3d-1$ and all possible messages sent as $t+1$ to Alice cause an expected update of $0.5$, so $\rho_t>3d-1.5 > 0.5-3\alpha$.}
            \subcase{$y_t=y, y'_t\neq y$.}
            {Then $d>\frac12-\alpha_t$. Bob's update with no corruption was expected to be $1$, Bob's actual update will be at least $3d-0.5$ and the message to Alice will cause an expected update of $0.5-0.5q_t=0.5-0.5(1-6d)=3d$, so $\rho_t>6d-1.5 > 1.5-6\alpha$. Notice that 
            }
            \end{subcaseof}
            If $y'_t=y$, then Bob's update will be at least $3d-1$ and all possible messages sent as $t+1$ to Alice cause an expected update of $0.5$, so their combined updates will be at least $3d-0.5$. If $y'_t\neq y$, Bob's expected update will be at least $3d-0.5$, but Alice's can be as low as 0. Thus, in either case, their expected updates will be at least $3d-0.5$. If $y_t=y$, then 
        }
        \end{caseof}
    \end{proof}
    
    \begin{caseof}
    \case{Bob does not know $x$ after message $2k-1$.}
    {
        \begin{subcaseof}
        \subcase{$(x_{2k-1},y_{2k-1},\delta_{2k-1})=(x_{2k-1},y_{2k-1},\delta_{2k-1})$ and $(x_{2k},y_{2k},\delta_{2k})=(x_{2k},y_{2k},\delta_{2k})$}
        {
            Then, Bob's chance of choosing the message changed from $0.5$ or $1$ to at least $0.5-3\alpha_{2k-1}$ or $1-3\alpha_{2k-1}$ respectively. In either case, this is a decrease of at most $3\alpha_{2k-1}$. The message either gains Bob 1 progress or 0 progress if chosen (since Alice will never send a message signaling a bad update) so the total expected progress only decreases by $3\alpha_{2k-1}$. The message Bob responds with will always be either $\ECC(\hat{x},y_{2k-1},?)$ or $\ECC(\hat{x},y,?)$. Since Bob is not right about $\hat{x}$, both of these would cause Alice to update 0.5 in expectation. Thus, 
        }
        \end{subcaseof}
    }
    \end{caseof}
    
    \begin{caseof}
        \case{Bob knows $x$ before receiving message $2k-1$.}{}
        \case{Bob does not know $x$ before receiving message $2k-1$ and does not know $x$ after receiving message $2k-1$.}
            {Then 
            \[
                \bbE [\Psi^A_k - \Psi^A_{k-1}] = \bbE [\psi_{2k}^A-\psi_{2k-2}^A] + \bbE [\psi_{2k}^B-\psi_{2k-2}^B].
            \]
            Let message $2k-1$ with no corruption be $\ECC(x_{2k-1},y_{2k-1},\delta_{2k-1})$.
            
            \begin{subcaseof} 
            \subcase{$y_{2k-1}\neq y$ (Alice does not know $y$).}
                {If $\alpha_{2k-1}\leq \frac13$, Bob's update in expectation can only decrease by $3\alpha$ since the update will happen with probability at least $\frac12-3\alpha$, and no update will happen the rest of the time. Bob will return either a response to Alice's real quesiton with an incorrect $x$, or $\ECC(?,y,0)$, both of which make Alice's expectation 0.5. }
            \end{subcaseof}
            }
    \end{caseof}
\end{proof}



==> x-one-way.tex <==
\section{One Way Communication over Binary Channels}

\begin{theorem}\cite{SpencerW92} \label{thm:three-liars}
    No interactive $1$-way protocol from Alice to Bob is resilient to an attack consisting of corrupting $\frac13$ of Alice's messages.
\end{theorem}

\input{one-way/2.7-upper}

\input{one-way/1.4-upper}




